HOIGS: Human-Object Interaction Gaussian Splatting

Reconstructing dynamic scenes with complex human-object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting methods either rely on human pose priors while neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. To address this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), which explicitly models interaction-induced deformation between humans and objects through a cross-attention-based HOI module. Distinct deformation baselines are employed to extract features: HexPlane for humans and Cubic Hermite Spline (CHS) for objects. By integrating these heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object manipulation. Comprehensive experiments on multiple datasets demonstrate that our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches, highlighting the importance of explicitly modeling human-object interactions for high-fidelity reconstruction.

==> tex_FIG/Intro_fig.tex <==
\maketitle
\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{images/intro/intro.jpg}
    % \vspace{-20pt}
    \caption{\textbf{Comparison between our method and previous approaches.}
    This figure compares rendering results between ExAvatar (\textcolor{blue}{\cite{moon2024expressive}}), a human-centric model, and Ex4DGS (\textcolor{blue}{\cite{lee2024fully}}), which uses a single motion field for all motions. ExAvatar reconstructs only humans, while Ex4DGS fails to represent contact in interaction scenarios, producing artifacts and noise around contact regions. }
    \label{fig:teaser}
\end{figure}
% \vspace{-10pt}

==> tex_FIG/intro_fig_explain_2.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/intro/intro.jpg}
    \vspace{-5mm}
    \caption{
    4DGS-based and human-centric model fail to render HOI scenes.
    }
    \label{fig:qualitative_hoi}
    \vspace{-7mm}
\end{figure}


==> tex_Tables/BEHAVE_Pose.tex <==
% \begin{table}[h]
% \centering
% \caption{
% Average quantitative evaluation on the BEHAVE dataset across all 8 scenes. The values correspond to \textbf{PA-MPJPE / PA-MPJPE (Hand/Forearm) / PA-PVE}. HOIGS demonstrates consistent average improvements over the baseline, particularly achieving a 6.1\% error reduction in the interaction-critical Hand/Forearm regions.
% }
% \label{tab:average_comparison}
% \def\arraystretch{1.4}
% \begin{tabular}{l|c}
% \specialrule{.1em}{.05em}{.05em}
% \textbf{Model} & \textbf{Average (All 8 scenes)} \\ \hline
% ExAvatar & 0.3034 / 0.3317 / 0.2795 \\
% HOIGS (Ours) & \textbf{0.2853} / \textbf{0.3114} / \textbf{0.2655} \\
% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}
% \vspace{2mm}
% \end{table}


% \begin{table}[t]
% \centering
% \caption{
% Quantitative evaluation on the BEHAVE dataset (averaged over 8 scenes).
% \textbf{PA-MPJPE}: pose error; \textbf{PA-MPJPE (H/F)}: hand/forearm region; \textbf{PA-PVE}: per-vertex error.
% }
% \label{tab:comparison}
% \small
% \setlength\tabcolsep{6pt}
% \def\arraystretch{1.3}
% \begin{tabular}{l|ccc}
% \specialrule{.1em}{.05em}{.05em}
% \textbf{Model} & \textbf{PA-MPJPE} & \textbf{PA-MPJPE (H/F)} & \textbf{PA-PVE} \\ \hline
% ExAvatar        & 0.3034 & 0.3317 & 0.2795 \\
% HOIGS (Ours)    & \textbf{0.2853} & \textbf{0.3114} & \textbf{0.2655} \\
% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}
% \end{table}
\begin{table}[t]
\setlength{\tabcolsep}{1pt}
\centering
\begin{minipage}{.48\linewidth}
\centering
\caption{Quantitative evaluation on the BEHAVE dataset (averaged over 8 scenes).
\textbf{PA-MPJPE}: pose error; \textbf{PA-MPJPE (H/F)}: hand/forearm region; \textbf{PA-PVE}: per-vertex error.
Per-scene results are provided in the supplementary material.}
\label{tab:behave_comparison}
\vspace*{-4mm}
\scalebox{0.7}{%
\begin{tabular}{C{2.8cm}|C{1.4cm}C{1.6cm}C{1.2cm}}
\specialrule{.1em}{.05em}{.05em}
Methods & PA-MPJPE\textdownarrow & PA-MPJPE (H/F)\textdownarrow & PA-PVE\textdownarrow \\ \hline
ExAvatar~\cite{moon2024exavatar}    & 0.3034 & 0.3317 & 0.2795 \\
\textbf{HOIGS (Ours)}              & \textbf{0.2853} & \textbf{0.3114} & \textbf{0.2655} \\
\specialrule{.1em}{.05em}{.05em}
\end{tabular}%
}
\end{minipage}%
\hspace{0.02\linewidth}%
\begin{minipage}{.48\linewidth}
\centering
\caption{Runtime performance comparison on the HOSNeRF dataset.
Our method maintains real-time performance ($>$30 FPS) despite the added complexity of interaction modeling.}
\label{tab:runtime_comparison}
\vspace*{-4mm}
\scalebox{0.7}{%
\begin{tabular}{C{3.0cm}|C{1.6cm}C{1.8cm}}
\specialrule{.1em}{.05em}{.05em}
Methods & Training Time & FPS\textuparrow \\ \hline
4DGS~\cite{wu20244d}               & 40 min      & 61.04 \\
Ex4DGS~\cite{lee2024fully}         & 2 hr 30 min & 46.38 \\
D3DGS~\cite{yang2024deformable}    & 3 hr        & 37.79 \\
E-D3DGS~\cite{bae2024per}          & 2 hr        & 54.71 \\ \hline
\textbf{HOIGS (Ours)}              & 5 hr        & 44.27 \\
\specialrule{.1em}{.05em}{.05em}
\end{tabular}%
}
\end{minipage}
\end{table}
% \begin{table*}[t]
% \centering
% \caption{
% Unified quantitative evaluation on the BEHAVE dataset.
% \textbf{PA-MPJPE}: pose error; \textbf{PA-MPJPE (H/F)}: hand/forearm region; \textbf{PA-PVE}: per-vertex error.
% HOIGS consistently outperforms the baseline across these metrics, particularly in interaction-critical regions.
% }
% \label{tab:unified_comparison}
% \small
% \setlength\tabcolsep{4pt}
% \def\arraystretch{1.3}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{C{2.5cm}|l|C{3.0cm}C{3.0cm}C{3.0cm}C{3.0cm}}
% \specialrule{.1em}{.05em}{.05em}
% % -------- Part 1: First 4 Classes --------
% \textbf{Model} & \textbf{Metric} &
% \textbf{Backpack\_1} &
% \textbf{Plasticcontainer\_1} &
% \textbf{Plasticcontainer\_2} &
% \textbf{Suitcase\_2} \\ \hline

% \multirow{3}{*}{ExAvatar}
%   & PA-MPJPE         & 0.4196 & 0.3875 & 0.3094 & 0.2654 \\
%   & PA-MPJPE (H/F)   & 0.4628 & 0.4282 & 0.3145 & 0.2957 \\
%   & PA-PVE           & 0.3687 & 0.3563 & 0.2897 & 0.2505 \\ \hline

% \multirow{3}{*}{HOIGS (Ours)}
%   & PA-MPJPE         & 0.4177 & 0.2964 & 0.2973 & 0.2438 \\
%   & PA-MPJPE (H/F)   & 0.4539 & 0.3344 & 0.3120 & 0.2649 \\
%   & PA-PVE           & 0.3656 & 0.2863 & 0.2837 & 0.2352 \\

% \specialrule{.1em}{.05em}{.05em}
% % -------- Part 2: Next 4 Classes --------
% \textbf{Model} & \textbf{Metric} &
% \textbf{Backpack\_3} &
% \textbf{Plasticcontainer\_3} &
% \textbf{Backpack\_6} &
% \textbf{Trashbin\_6} \\ \hline

% \multirow{3}{*}{ExAvatar}
%   & PA-MPJPE         & 0.2690 & 0.3293 & 0.2177 & 0.2294 \\
%   & PA-MPJPE (H/F)   & 0.3135 & 0.3298 & 0.2494 & 0.2597 \\
%   & PA-PVE           & 0.2488 & 0.2970 & 0.2092 & 0.2156 \\ \hline

% \multirow{3}{*}{HOIGS (Ours)}
%   & PA-MPJPE         & 0.2629 & 0.3270 & 0.2110 & 0.2263 \\
%   & PA-MPJPE (H/F)   & 0.3068 & 0.3265 & 0.2380 & 0.2550 \\
%   & PA-PVE           & 0.2438 & 0.2948 & 0.2020 & 0.2126 \\

% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}%
% }
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{
% Unified quantitative evaluation on the BEHAVE dataset. The values in each cell correspond to \textbf{PA-MPJPE / PA-MPJPE (Hand/Forearm) / PA-PVE}. HOIGS consistently outperforms the baseline across these metrics, particularly in interaction-critical regions.
% }
% \label{tab:unified_comparison}
% \small  % \tiny 대신 \small 사용
% \setlength\tabcolsep{3.0pt}  % 여백 살짝 증가
% \def\arraystretch{1.4}
% % \resizebox 제거 → 글자 크기가 실제로 반영됨
% \begin{tabular}{C{2.8cm}|C{3.5cm}C{3.5cm}C{3.5cm}C{3.5cm}}
% \specialrule{.1em}{.05em}{.05em}

% % -------- Part 1: First 4 Classes --------
% \textbf{Model} &
% \textbf{Backpack1} &
% \textbf{Plasticcontainer1} &
% \textbf{Plasticcontainer2} &
% \textbf{Suitcase1} \\ \hline

% ExAvatar & 
% 0.4196 / 0.4628 / 0.3687 & 
% 0.3875 / 0.4282 / 0.3563 & 
% 0.3094 / 0.3145 / 0.2897 & 
% 0.2654 / 0.2957 / 0.2505 \\

% HOIGS (Ours) & 
% 0.4177 / 0.4539 / 0.3656 & 
% 0.2964 / 0.3344 / 0.2863 & 
% 0.2973 / 0.3120 / 0.2837 & 
% 0.2438 / 0.2649 / 0.2352 \\

% \specialrule{.1em}{.05em}{.05em}

% % -------- Part 2: Next 4 Classes --------
% \textbf{Model} &
% \textbf{Backpack2} &
% \textbf{Plasticcontainer3} &
% \textbf{Backpack3} &
% \textbf{Trashbin} \\ \hline

% ExAvatar & 
% 0.2690 / 0.3135 / 0.2488 & 
% 0.3293 / 0.3298 / 0.2970 & 
% 0.2177 / 0.2494 / 0.2092 & 
% 0.2294 / 0.2597 / 0.2156 \\

% HOIGS (Ours) & 
% 0.2629 / 0.3068 / 0.2438 & 
% 0.3270 / 0.3265 / 0.2948 & 
% 0.2110 / 0.2380 / 0.2020 & 
% 0.2263 / 0.2550 / 0.2126 \\

% \specialrule{.1em}{.05em}{.05em}

% \end{tabular}
% \end{table*}

==> tex_Tables/ablation.tex <==
\begin{table}[t!]
    \centering
    \caption{Ablation studies on the HOSNeRF dataset using our method. The \textbf{best} results are highlighted.}
    \label{ablation}
    \scalebox{0.75}{
    \begin{tabular}{l|cc}
        \hline
        \multirow{}{}{} & \multicolumn{2}{c}{Avg (6 scenes)} \\
        & PSNR$\uparrow$ & LPIPS$\downarrow$ \\
        \hline
        w/o CHS deformation (using MLP) & 24.52 & 0.154 \\
        Baseline deformation             & 25.01 & 0.130 \\
        w/o human feature                & 25.67 & 0.119 \\
        w/o HOI module                   & 25.24 & 0.128 \\
        \rowcolor{gray!15}
        HOIGS (\textbf{Ours})            & \textbf{25.89} & \textbf{0.114} \\
        \hline
    \end{tabular}}
\end{table}


==> tex_main/0_Abstract.tex <==
% \begin{abstract% }
%Reconstructing human-object interaction scenes from monocular videos in the wild remains a significant challenge due to the absence of reliable 3D priors and complex dynamic motions. Existing human-centric reconstruction methods rely heavily on accurate human pose priors and struggle with general dynamic objects, while 4D Gaussian Splatting approaches often fail to capture detailed object motion under occlusion or during long sequences. We present HOIGS, a novel framework that jointly reconstructs humans, dynamic objects, and backgrounds using 3D Gaussians in a unified world space. Our method leverages Score Distillation Sampling (SDS) from a pretrained diffusion model to generate complete 360\textdegree{} 3D shapes at key frames, providing strong geometric priors for initializing dynamic object Gaussians. These priors are temporally propagated using cubic hermite splines, enabling smooth and continuous deformation across time while refining alignment across frames. By combining SMPL-based human modeling, spline-based dynamic object tracking, and Gaussian-based scene representation, HOIGS achieves high-quality reconstruction of complex interaction scenes from monocular inputs. We demonstrate the effectiveness of our approach on challenging real-world sequences, showing substantial improvements over existing baselines in both geometric accuracy and visual fideli% ty.
%\end{abstract}

\begin{abstract}
%인간–객체 상호작용이 포함된 동적 장면을 재구성하는 것은 컴퓨터 비전과 그래픽스 분야의 근본적인 도전 과제이다. 기존 Gaussian Splatting 기반 방법들은 인간 포즈 사전정보에 의존하여 동적 객체를 간과하거나, 모든 움직임을 단일 motion field로 근사하여 복잡한 상호작용을 충분히 포착하지 못한다. 이를 해결하기 위해 본 연구에서는 인간과 객체 간 motion consistency를 명시적으로 학습하는 Human-Object Interaction Gaussian Splatting (HOIGS)를 제안한다. HOIGS는 cross-attention 기반의 HOI 모듈을 통해 사람과 객체의 motion feature 간 상호 의존성을 효과적으로 학습하며, 사람에 대해서는 HexPlane, 객체에 대해서는 Cubic Hermite Spline (CHS)을 deformation baseline으로 적용하여 상호 보완적인 motion feature를 추출한다. 이러한 특징을 통해 HOIGS는 occlusion, contact, manipulation과 같은 복잡한 상호작용 상황에서도 보다 정밀한 deformation 추정을 가능하게 한다. 다양한 데이터셋에서의 실험 결과, 제안한 방법은 기존 human-centric 및 4D Gaussian 접근법을 안정적으로 능가하며, 상호작용 장면의 고품질 재구성을 위한 새로운 가능성을 보여준다.
% Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. To address this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), which explicitly models interaction-induced deformation between humans and objects through a cross-attention based HOI module. Distinct deformation baselines are employed to extract complementary motion features: HexPlane for humans and Cubic Hermite Spline (CHS) for objects. By integrating these heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object manipulation. Comprehensive experiments on multiple datasets demonstrate that our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches, highlighting the importance of explicitly modeling human–object interactions for high-fidelity reconstruction. The video results of HOIGS are available at: \url{https://anonymous.4open.science/w/HOI-GS/}



% Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. To address this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), which explicitly models interaction-induced deformation between a human and multiple objects through a cross-attention based HOI module. Distinct deformation baselines are employed to extract complementary motion features: HexPlane for the human and Cubic Hermite Spline (CHS) for objects. By integrating these heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object manipulation. Comprehensive experiments on multiple datasets demonstrate that our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches. The video results of HOIGS are available at: \url{https://anonymous.4open.science/w/HOI-GS/}



% Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. To address this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), which explicitly models interaction-induced deformation between humans and objects through a cross-attention based HOI module. Distinct deformation baselines are employed to extract complementary motion features: HexPlane for humans and Cubic Hermite Spline (CHS) for objects. By integrating these heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object manipulation. Comprehensive experiments on multiple datasets demonstrate that our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches, highlighting the importance of explicitly modeling human–object interactions for high-fidelity reconstruction. Video results demonstrating the effectiveness of our method are available in the supplementary material.




Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting
methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. To address this gap, we propose Human-Object Interaction Gaussian
Splatting (HOIGS), which explicitly models interaction-induced deformation between humans and objects through a cross-attention based HOI module. Distinct
deformation baselines are employed to extract complementary motion features: HexPlane for humans and Cubic Hermite Spline (CHS) for objects. By integrating these
heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object
manipulation. Comprehensive experiments on multiple datasets demonstrate that
our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches, highlighting the importance of explicitly modeling human–object
interactions for high-fidelity reconstruction. The video results of HOIGS are available at: \url{https://anonymous.4open.science/w/HOIGS-0F47/} 
% Video results demonstrating the effectiveness of our method are available in the supplementary material.
\keywords{Human-Object Interaction (HOI) \and Gaussian Splatting \and Dynamic Scene Reconstruction}




% Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. \textcolor{blue}{To address this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), which explicitly models interaction-induced deformation between a human and multiple objects through a cross-attention based HOI module.} \textcolor{blue}{Distinct deformation baselines are employed to extract complementary motion features: HexPlane for the human and Cubic Hermite Spline (CHS) for objects.} By integrating these heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object manipulation. \textcolor{blue}{Comprehensive experiments on multiple datasets demonstrate that our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches.} \textcolor{blue}{The video results of HOIGS are available at: \url{https://anonymous.4open.science/w/HOI-GS/}}




\end{abstract}

==> tex_main/0_Abstract_1.tex <==
% Alternative Version with Different Emphasis
% This version emphasizes the technical innovation more strongly

\begin{abstract}
Reconstructing dynamic scenes with complex human--object interactions from monocular video remains a fundamental challenge in computer vision. 
%
While recent Gaussian Splatting methods have shown promise, they either focus solely on humans using pose priors, neglecting object dynamics, or treat all motions uniformly within a single deformation field, failing to capture the rich interdependencies inherent in human--object interactions.
%
We present \textit{Human-Object Interaction Gaussian Splatting} (HOIGS), a novel framework that explicitly disentangles and models the coupled deformation between humans and objects.
%
Our key contribution is a unified representation that combines entity-specific motion priors—HexPlane-based features for articulated human deformation and Cubic Hermite Spline parameterization for smooth object trajectories—with a cross-attention interaction module that learns their mutual influence.
%
This design enables HOIGS to accurately reconstruct challenging scenarios involving occlusion, contact, and manipulation from monocular input.
%
Extensive experiments demonstrate that HOIGS consistently surpasses state-of-the-art human-centric and 4D Gaussian approaches across multiple benchmarks, establishing the effectiveness of explicit interaction modeling for high-fidelity dynamic scene reconstruction.
%
Video results: \url{https://anonymous.4open.science/w/HOIGS-0F47/}
\end{abstract}

\keywords{Human-Object Interaction \and Gaussian Splatting \and Dynamic Scene Reconstruction}

==> tex_main/1_Introduction.tex <==
\section{Introduction}

%1. 논문에서 다루고자 하는 task (task의 중요성 설명)
% 복잡한 인간–객체 상호작용이 포함된 장면의 비디오를 재구성하고 새로운 시점을 합성하는 것은 컴퓨터 비전과 그래픽스 분야에서 핵심적인 연구 주제이다. 이러한 기술은 가상현실, 메타버스, 3D 애니메이션 등 다양한 응용으로 확장될 수 있다. 그러나 단일 시점 카메라의 한계와 인간–객체 간의 복잡한 상호작용을 정확히 모델링해야 한다는 점은 여전히 고품질 재구성을 위한 주요 도전 과제로 남아 있다. 이러한 문제를 해결하는 것은 실제와 유사한 장면의 이해와 표현을 가능하게 하는 데 필수적이다.

Reconstructing videos of scenes that involve complex interactions between humans and objects and synthesizing novel viewpoints constitute a central research problem in computer vision and graphics. These techniques can be extended to various applications, including virtual reality, the metaverse, and 3D animation. However, the inherent limitations of monocular cameras and the need to accurately model intricate interactions between humans and objects remain major challenges for achieving high-quality reconstruction. Addressing these issues is essential for enabling realistic scene understanding and representation.  


%2. 해당 task의 기존 연구들 -> 문제점을 함꼐 언급하면서 진행

% 2-1 Human 기반의 Gaussian Splatting 기반 문제점을 언급

%최근 사람 중심 비디오 장면 재구성 연구들은 Human Pose Estimation과 Gaussian Splatting을 결합하여 모델링을 수행한다. 일반적으로 각 프레임에 대해 회귀된 SMPL 파라미터를 사전에 획득한 뒤, T-pose를 기준으로 canonical space를 정의하고, 해당 공간에서 3D Gaussian 파라미터를 설정한다. 이후 feature plane과 MLP를 통해 해당 파라미터를 학습하고, LBS(linear blend skinning) 함수를 이용하여 각 프레임에 해당하는 3D 공간으로의 deformation을 적용함으로써 전체 장면을 구성하고 렌더링한다. 이러한 방식은 사람과 배경에 특화된 모델로 발전해왔으며, 정밀한 human pose 정보에 기반해 상대적으로 안정적인 성능을 보인다.
%그러나 기존 접근법들은 사람의 자세 정보를 중심으로 설계되어 있어, 사람과 객체가 동시에 상호작용하는 장면을 직접적으로 모델링하지 못한다. 이로 인해 객체가 동적으로 움직이는 경우에도 정적인 배경으로 처리되거나, 상호작용 과정에서 사람과 객체 간의 관계가 충분히 반영되지 않는 한계가 있다. 따라서 사람과 객체가 함께 상호작용하는 장면을 정확히 재구성하기 위해서는 기존 human-centric 모델을 넘어서는 새로운 모델링 방식이 요구된다.

Recent approaches on human-centric video scene reconstruction (\textcolor{blue}{\cite{kocabas2024hugs,moon2024expressive,hu2024gauhuman,qian20243dgs, liu2024animatable, hu2024gaussianavatar, wen2024gomavatar, kim2025showmak3r}}) have combined human pose estimation with 3D Gaussian Splatting (3DGS) (\textcolor{blue}{\cite{kerbl20233d}}) to model dynamic scenes. Typically, SMPL (\textcolor{blue}{\cite{loper2023smpl}}) parameters are regressed in advance for each frame, and a canonical space is defined using a T-pose as the reference. Within this space, 3D Gaussian parameters are established and trained using feature planes and MLPs. Subsequently, deformation to each frame's 3D space is performed via Linear Blend Skinning (LBS) (\textcolor{blue}{\cite{loper2023smpl}}), allowing for scene reconstruction and rendering. These methods have evolved into specialized models focused on humans and static backgrounds, achieving reliable performance when accurate human pose priors are available. However, existing approaches mainly focus on modeling humans alone, and thus fail to reconstruct complete scenes that involve objects beyond the human body. As a result, dynamically moving objects are often treated as static background or even disappear from the reconstructed scene. Even when deformations of objects are modeled separately, the interactions between humans and objects are not sufficiently considered in dynamic scenarios, which leads to artifacts and noisy results in the interaction regions, as shown in Fig. \textcolor{blue}{\ref{fig:teaser}}. Consequently, accurately reconstructing scenes that involve both humans and objects requires new modeling paradigms that extend beyond conventional human-centric frameworks.

% 2-2 Dynamic scene을 대상으로하흔 Gaussian Splatting의 문제점 언급

%4D Gaussian Splatting 기반 연구들은 사람에 한정되지 않고 임의의 움직이는 객체까지 포괄할 수 있다는 장점이 있으나, 사람 중심 모델에 비해 인간 재구성 성능은 떨어지는 경향이 있다. 이러한 연구들은 대체로 canonical space를 정의하고 이를 world coordinate로 deform하는 implicit function을 학습하거나, 객체의 움직임을 explicit하게 파라미터화하여 학습하는 방식으로 발전하고 있다. 그러나 이러한 접근법들은 객체 간 상호작용을 명시적으로 모델링하지 않고, 모든 움직이는 객체를 단일 motion field로 다루기 때문에 복잡한 interaction을 충분히 반영하지 못한다. 그 결과 implicit 방식은 장기간 혹은 비선형적인 동작을 안정적으로 표현하기 어렵고, explicit 방식은 occlusion, contact, object-to-object dynamics와 같이 interaction에 따라 변화하는 다양한 시나리오를 포괄하기 어렵다.

Recent studies on 4D Gaussian Splatting extend beyond humans to encompass arbitrary moving objects, offering the advantage of general applicability. However, they generally exhibit lower reconstruction performance for humans compared to human-centric models. These approaches typically either define a canonical space and learn an implicit function that deforms it into the world coordinate system (\textcolor{blue}{\cite{wu20244d,jung2023deformable,bae2024per}}), or explicitly parameterize object motions and optimize the corresponding parameters (\textcolor{blue}{\cite{yang2023real,li2024spacetime,lee2024fully}}). Nevertheless, they do not explicitly model interactions between objects and instead treat all moving entities within a single motion field, which limits their ability to capture complex interactions. As a result, implicit methods struggle to represent long-term or highly non-linear motions in a stable manner, while explicit methods fail to handle scenarios such as contact and object manipulation, as ignoring the mutual interactions between motions limits their ability to capture realistic dynamics.

%3. 해당 문제를 해결하기위한 우리의 제안 방법 
%이러한 한계를 극복하기 위해, 우리는 Human-Object Interaction Gaussian Splatting (HOIGS)를 제안한다. HOIGS는 사람과 동적 객체가 동시에 등장하는 복잡한 비디오 장면을 재구성하기 위한 통합 프레임워크로, 기존 접근법이 주로 사람의 움직임만을 모델링했던 것과 달리 사람–객체 간 상호작용을 명시적으로 고려하여 보다 정밀한 deformation 모델링을 가능하게 한다.

%우리 방법의 핵심은 HOI module이며, 이 모듈은 mutual attention 구조를 통해 각 프레임에서 사람의 feature와 객체의 motion feature 간의 양방향 의존성을 학습한다. 구체적으로, 사람의 경우 HexPlane 표현에서 시간에 따라 변화하는 성분을 활용하고, 객체의 경우 keyframe Gaussian의 velocity vector와 관련 파라미터를 임베딩하여 motion feature를 추출한다. 이렇게 얻어진 두 feature를 상호작용하는 attention 구조로 학습함으로써, 기존 연구들이 사람과 객체를 독립적으로 모델링함에 따라 발생했던 artifact나 불안정한 재구성 문제를 효과적으로 해결한다.

%또한, 우리는 사람과 객체 각각에 적합한 deformation baseline을 도입하였다. 객체의 경우, Cubic Hermite Spline (CHS)를 활용하여 연속적인 motion trajectory를 표현하고, keyframe Gaussian의 velocity vector와 추가적인 학습 가능한 파라미터를 결합하여 강건한 motion feature를 형성한다. 사람의 경우에는 HexPlane을 deformation baseline으로 사용하여, 시간적으로 변화하는 파라미터를 공간 feature와 함께 활용함으로써 세밀한 사람의 변형을 효과적으로 모델링한다. 이렇게 추출된 사람과 객체의 feature는 HOI module에 통합되어 각각의 offset vector를 출력하게 되며, 이를 통해 접촉, 조작(manipulation), 복잡한 상호작용 등 다양한 시나리오에서도 정확하고 안정적인 deformation 추정이 가능하다.

To overcome these limitations, we propose Human-Object Interaction Gaussian Splatting (HOIGS), a unified framework for reconstructing complex video scenes that involve both humans and dynamic objects. Unlike previous approaches that either model only human motion or employ a single motion field for all entities, our framework explicitly incorporates human–object interactions to achieve more faithful deformation modeling.

% \textcolor{blue}{
% We introduce deformation baselines tailored to the distinct characteristics of humans and objects. For humans, we employ SMPL-X-based Gaussian modeling to achieve robust representation against occlusions and detailed deformation. By combining temporally varying parameters with spatial features, we effectively model fine-grained human deformation while maintaining inter-frame consistency. For objects, we apply Cubic Hermite Spline (CHS) to smoothly represent continuous motion trajectories, forming robust motion feature representations by combining velocity vectors of keyframe Gaussians with learnable auxiliary parameters.
% }
% \textcolor{blue}{
% Finally, we design a Cross-Attention-based HOI module to reflect interaction intensity between humans and multiple objects. Extracted human features and object features exchange information complementarily through cross-attention, generating interaction features. Subsequently, through MLP heads, Gaussian mean offsets are predicted for objects, while SMPL-X pose offsets are predicted for humans. This interaction-based attention architecture enables accurate and stable deformation estimation across diverse scenarios including artifacts, contact, manipulation, occlusion, and complex interactions that arise when modeling humans and objects independently.
% }
At the core of our framework lies the HOI module, which adopts a mutual attention mechanism to capture the bidirectional dependencies between human features and object motion features at each frame. Specifically, the module receives temporally varying human features, derived from the dynamic components of the HexPlane representation, together with object motion features, obtained by embedding velocity vectors and their associated parameters. By explicitly learning how these two types of features influence one another, the HOI module effectively overcomes the shortcomings of prior methods that modeled humans and objects independently, which often resulted in artifacts and unstable reconstructions in interaction-rich scenes.

Furthermore, we design different deformation baselines tailored to humans and objects. For objects, we employ the Cubic Hermite Spline (CHS) to capture continuous motion trajectories, embedding the velocity vectors of keyframe Gaussians along with additional learnable parameters to construct robust object motion features. For humans, we utilize HexPlane as the deformation baseline, where time-varying parameters are leveraged to represent fine-grained human deformation in both spatial and temporal domains. The extracted features from both humans and objects are subsequently integrated within the HOI module, which outputs offset vectors for each entity. This design ultimately enables our framework to achieve accurate and stable deformation estimation, even under complex scenarios involving close contact, mutual manipulation, or other intricate human–object interactions.

In summary, our main contributions are as follows:

\begin{itemize}
 
    \item We propose an entity-aware cross-attention HOI module that enforces motion consistency between humans and objects. By attending to their features, it captures interdependent dynamics and improves reconstruction during contact and manipulation.
        
    \item We design distinct strategies for humans and objects using tailored deformation baselines. HexPlane encodes temporal and spatial features for human motion, while Cubic Hermite Splines (CHS) embed velocity vectors and learnable parameters for objects. This separation enables accurate and expressive motion representations for both entities.

    \item We conduct extensive experiments on diverse human–object interaction scenes and demonstrate that our method achieves more accurate reconstruction compared to existing human-centric and 4D Gaussian approaches.

\end{itemize} 

==> tex_main/1_Introduction_revised.tex <==
\section{Introduction}

Reconstructing dynamic scenes featuring complex human-object interactions from monocular videos, alongside synthesizing novel viewpoints, is a fundamental challenge in computer vision and graphics. High-fidelity reconstruction of such interactive scenes is essential for unlocking immersive applications in virtual reality, 3D animation, and the metaverse. However, achieving photorealistic and physically plausible reconstructions remains immensely challenging due to the inherent ambiguities of monocular capture and the intricate, mutually dependent dynamics between humans and objects. Addressing these issues is essential for enabling realistic scene understanding and representation.
+4

Recent human-centric dynamic scene reconstruction methods (\cite{kocabas2024hugs,moon2024expressive,hu2024gauhuman,qian20243dgs, liu2024animatable, hu2024gaussianavatar, wen2024gomavatar, kim2025showmak3r}) have successfully coupled human pose priors, such as the SMPL model (\cite{loper2023smpl}), with 3D Gaussian Splatting (3DGS) (\cite{kerbl20233d}). These approaches typically establish a canonical space based on a reference T-pose, optimize 3D Gaussian parameters using feature planes and MLPs, and deform them into the observation space via Linear Blend Skinning (LBS) (\cite{loper2023smpl}). While these methods achieve reliable performance for human bodies and static backgrounds, they fundamentally lack the capacity to explicitly model dynamic objects. Consequently, interacting objects are either erroneously baked into the static background or entirely omitted. Even when object deformations are treated separately, the failure to model the explicit coupling between humans and objects yields severe artifacts and noisy reconstructions in interaction-rich regions (see Fig. \ref{fig:teaser}). Accurately reconstructing scenes that involve both humans and objects requires new modeling paradigms that extend beyond conventional human-centric frameworks.
+4

Conversely, general dynamic scene reconstruction methods based on 4D Gaussian Splatting (4DGS) extend beyond humans to encompass arbitrary moving entities. These approaches generally define an implicit deformation field that warps a canonical space into world coordinates (\cite{wu20244d,jung2023deformable,bae2024per}), or explicitly parameterize and optimize object motions (\cite{yang2023real,li2024spacetime,lee2024fully}). Nevertheless, they typically subsume all moving entities into a single, global motion field, completely ignoring the explicit physical interactions between them. As a result, implicit methods struggle to stabilize long-term or highly non-linear trajectories, while explicit parameterizations falter under complex interaction scenarios like contact, occlusion, and object manipulation. Furthermore, their human reconstruction fidelity noticeably lags behind that of specialized human-centric models.
+4

To bridge this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), a unified framework explicitly designed to reconstruct complex monocular videos featuring interacting humans and dynamic objects. Unlike previous paradigms that isolate human motion or oversimplify scenes into a unified motion field, our method explicitly disentangles human and object representations while enforcing their interdependencies. At the core of our framework is the Cross-Attention Human-Object Interaction (HOI) module, which employs a mutual attention mechanism to capture bidirectional dependencies at every frame. By explicitly computing the attention between temporally varying human features and object motion features, the HOI module effectively resolves the artifacts and temporal instabilities that plague independent modeling approaches during close-contact interactions.
+4

Recognizing the distinct dynamic characteristics of humans and rigid objects, we introduce tailored deformation baselines to extract robust features for the HOI module. For objects, we adopt a Cubic Hermite Spline (CHS) to model smooth, continuous motion trajectories. By embedding the velocity vectors of keyframe Gaussians alongside learnable auxiliary parameters, we construct a highly expressive object motion feature representation. For humans, we employ a HexPlane-based deformation field, leveraging time-varying parameters to capture fine-grained spatial and temporal human deformations. The heterogeneous features extracted from these independent baselines are integrated into the HOI module, which outputs interaction-aware offset vectors for both entities. This synergistic design ensures accurate and stable deformation estimation, even under intricate scenarios involving mutual manipulation, occlusion, and sustained contact.
+4

In summary, our main contributions are as follows:
\begin{itemize}
\item We propose HOIGS, a novel framework featuring an entity-aware cross-attention HOI module that explicitly enforces motion consistency between humans and objects. By attending to their features, it captures interdependent dynamics and significantly improves reconstruction fidelity during complex interactions, contact, and manipulation. \item We design distinct, highly tailored deformation baselines for humans and objects. We utilize HexPlane representations to encode spatiotemporal human motion, and Cubic Hermite Splines (CHS) with embedded velocity vectors and learnable parameters to capture robust object trajectories. This separation enables accurate and expressive motion representations for both entities. \item Extensive experiments on diverse human-object interaction scenes demonstrate that HOIGS achieves superior reconstruction accuracy and rendering quality compared to state-of-the-art human-centric and 4D Gaussian approaches. 
\end{itemize}

==> tex_main/1_Introduction_revised_3.tex <==
\section{Introduction}

Reconstructing dynamic scenes involving complex human--object interactions from monocular videos is a fundamental challenge in computer vision and graphics. Such capabilities are essential for applications in virtual reality, metaverse experiences, and 3D animation. However, the inherent constraints of monocular capture and the difficulty of accurately modeling intricate human--object interactions pose significant obstacles to achieving high-fidelity reconstruction.

Recent human-centric methods~\cite{kocabas2024hugs,moon2024expressive,hu2024gauhuman,qian20243dgs,liu2024animatable,hu2024gaussianavatar,wen2024gomavatar,kim2025showmak3r} have made substantial progress by combining human pose estimation with 3D Gaussian Splatting (3DGS)~\cite{kerbl20233d}. These approaches typically regress SMPL parameters~\cite{loper2023smpl} for each frame, define a canonical T-pose space, and train 3D Gaussian parameters using feature planes and MLPs. Deformation to each frame is achieved via Linear Blend Skinning (LBS)~\cite{loper2023smpl}, enabling photorealistic rendering. While these specialized models perform reliably when accurate human pose priors are available, they predominantly focus on modeling humans alone. Consequently, dynamic objects are often treated as static background elements or disappear entirely from reconstructed scenes. Even when object deformations are modeled separately, the lack of explicit interaction modeling between humans and objects leads to artifacts and noisy results in contact regions, as illustrated in Fig.~\ref{fig:teaser}.

An alternative line of work based on 4D Gaussian Splatting extends modeling to arbitrary moving objects~\cite{wu20244d,jung2023deformable,bae2024per,yang2023real,li2024spacetime,lee2024fully}. These methods either define a canonical space and learn implicit deformation functions to the world coordinate system, or explicitly parameterize object motions and optimize the corresponding parameters. Despite their generality, these approaches typically exhibit lower reconstruction quality for humans compared to human-centric models. More critically, they treat all moving entities within a single motion field without explicitly modeling object interactions. This limitation hinders their ability to capture complex dynamics: implicit methods struggle with long-term or highly non-linear motions, while explicit methods fail to handle scenarios involving contact, occlusion, and object manipulation.

To address these limitations, we propose \textbf{Human-Object Interaction Gaussian Splatting (HOIGS)}, a unified framework that explicitly models human--object interactions for high-fidelity reconstruction of dynamic scenes from monocular videos. Unlike prior work that either focuses solely on humans or treats all entities within a unified motion field, our approach captures the bidirectional dependencies between human and object motions through a dedicated interaction module.

At the core of HOIGS lies a cross-attention-based HOI module that captures the interdependencies between human and object features at each frame. For humans, we extract temporally varying features from a HexPlane representation, while for objects, we construct motion features by embedding velocity vectors and learnable parameters. Through mutual attention, the HOI module learns how these features influence each other, effectively addressing the artifacts and instabilities that arise when humans and objects are modeled independently.

We further design distinct deformation baselines tailored to the characteristics of each entity. For objects, we employ Cubic Hermite Splines (CHS) to model continuous motion trajectories, incorporating velocity vectors of keyframe Gaussians with additional learnable parameters. For humans, we leverage HexPlane-based features with time-varying parameters to capture fine-grained spatial and temporal deformations. The extracted features are integrated within the HOI module to predict entity-specific offset vectors, enabling accurate deformation estimation even in complex scenarios involving close contact, manipulation, and occlusion.

Our main contributions are as follows:
\begin{itemize}
    \item We propose an entity-aware cross-attention HOI module that enforces motion consistency between humans and objects, capturing interdependent dynamics to improve reconstruction quality during contact and manipulation.
        
    \item We design distinct deformation strategies tailored to humans and objects: HexPlane-based features for spatial-temporal human motion, and Cubic Hermite Splines with embedded velocity vectors for smooth object trajectories. This separation enables accurate and expressive motion representations for both entities.

    \item We conduct extensive experiments on diverse human--object interaction datasets, demonstrating that our method achieves superior reconstruction quality compared to state-of-the-art human-centric and 4D Gaussian approaches.
\end{itemize}


==> tex_main/2_Realatedwork_revised.tex <==
\section{Related Works}

\subsection{3D Human Modeling}
The reconstruction of digital humans has evolved significantly, progressing from parametric estimations to high-fidelity volumetric representations. Early approaches relied on parametric models to efficiently estimate human pose and shape, as exemplified by HMR \cite{kanazawa2018end}. However, these methods often struggle to capture surface details such as clothing and accessories. To overcome these limitations, implicit function-based methods \cite{huang2020arch, saito2019pifu, saito2020pifuhd, xiu2022icon, xiu2023econ} were introduced to recover fine-grained geometry, though they frequently lack global consistency and rendering efficiency.

Following the success of Neural Radiance Fields (NeRF) \cite{mildenhall2021nerf}, numerous works adapted volumetric rendering for human modeling \cite{peng2021neural, jiang2022neuman, weng2022humannerf, alldieck2022photorealistic, liao2023high, guo2023vid2avatar}, achieving impressive appearance fidelity and view consistency. Despite these advancements, NeRF-based methods generally suffer from high training costs and slow inference speeds. In the context of Human-Object Interaction (HOI), methods like HOLD \cite{fan2024hold} have attempted to introduce objects into the reconstruction pipeline, yet they often fail to fully capture the dynamic interplay between the human and the object.

Most recently, 3D Gaussian Splatting (3DGS) \cite{kerbl20233d} has emerged as a powerful alternative, enabling real-time rendering and high-quality reconstruction. This representation has been rapidly adopted for human avatars \cite{kocabas2024hugs, moon2024expressive, hu2024gauhuman, liu2024animatable, hu2024gaussianavatar}. Nevertheless, the majority of these human-centric approaches treat interacted objects as static background elements or ignore them entirely. While recent multi-view approaches such as Animatable Gaussian \cite{li2024animatable} and GASPACHO \cite{mir2025gaspacho} have successfully disentangled human-object interactions to create relightable avatars, they rely on complex multi-camera setups. In contrast, real-world applications often demand robust performance from monocular inputs. To address this, we propose HOIGS, a unified framework that explicitly models dynamic human-object interactions from monocular video, ensuring stability and physical plausibility.

\subsection{Dynamic Scene Modeling}
The paradigm of dynamic scene reconstruction has shifted from implicit neural fields to explicit Gaussian-based representations. Initial dynamic scene methods extended NeRF to the temporal domain \cite{park2021nerfies, park2021hypernerf, wu2022d, fridovich2023k}. Within this category, HOSNeRF \cite{liu2023hosnerf} notably attempted to model HOI scenarios by controlling human motion via skeleton-based priors (SMPL) and incorporating object state embeddings. However, the implicit nature of these representations incurs significant computational overhead and limits the ability to resolve high-frequency details in large-scale dynamic environments.

To mitigate these efficiency bottlenecks, recent works have extended 3DGS to 4D Gaussian Splatting (4DGS) \cite{wu20244d, yang2023real}. Although 4DGS achieves real-time rendering, it faces two fundamental challenges when applied to complex interaction scenarios. First, most 4DGS approaches rely on Structure-from-Motion (SfM) for initialization. SfM assumes a static world, making it inherently ill-suited for initializing points on moving objects, leading to inaccurate geometry. Second, these methods typically employ MLP-based implicit deformation fields to model motion. While sufficient for simple trajectories, implicit fields tend to over-smooth complex, non-linear movements, resulting in unnatural dynamics during intricate interactions.

To overcome these limitations, we propose an explicit, spline-based motion model. By eschewing implicit deformation fields in favor of explicit trajectory modeling, our approach captures intricate temporal movements with high fidelity, enabling high-quality rendering of dynamic scenes characterized by complex human-object interactions.

==> tex_main/2_Realatedwork_revised_2.tex <==
\section{Related Works}

\subsection{3D Human Modeling and Interaction}
\noindent\textbf{3D Human Avatars.}
Research on realistic human modeling has evolved significantly from parametric estimation to neural implicit representations. 
Early approaches relied on parametric models like SMPL to estimate pose and shape \cite{kanazawa2018end}, yet these methods often struggle to capture surface details such as loose clothing. 
To address this, implicit function-based methods \cite{huang2020arch, saito2019pifu, saito2020pifuhd, xiu2022icon, xiu2023econ} were proposed to recover fine-grained geometry, though they frequently lack global consistency and suffer from slow inference speeds. 
The advent of Neural Radiance Fields (NeRF) \cite{mildenhall2021nerf} enabled high-fidelity view synthesis for human avatars \cite{peng2021neural, jiang2022neuman, weng2022humannerf, alldieck2022photorealistic, liao2023high, guo2023vid2avatar}; however, the high computational cost of volumetric rendering limits their real-time applicability.
Most recently, 3D Gaussian Splatting (3DGS) \cite{kerbl20233d} has emerged as a powerful alternative, offering real-time rendering with explicit geometry control. 
Several works have successfully adapted 3DGS for human reconstruction \cite{kocabas2024hugs, moon2024expressive, hu2024gauhuman, liu2024animatable, hu2024gaussianavatar}, utilizing LBS-based deformation or learned feature planes to animate human subjects. 
Despite these advancements, the majority of these frameworks treat the scene as strictly human-centric, often regarding interacting objects as static background or ignoring them entirely, which leads to severe artifacts in dynamic interaction scenarios.

\noindent\textbf{Human-Object Interaction Reconstruction.}
While human modeling has matured, reconstructing dynamic human-object interactions (HOI) remains a nascent challenge. 
Early attempts introduced object templates into the optimization pipeline \cite{fan2024hold}, yet often failed to fully capture the coupled dynamics of the interaction. 
HOSNeRF \cite{liu2023hosnerf} made a significant step by modeling interactions through object state embeddings and skeleton-driven deformations; however, its reliance on implicit NeRF representations results in significant training overhead and difficulties in scaling to large environments.
More recent multi-view approaches, such as Animatable Gaussian \cite{li2024animatable} and GASPACHO \cite{mir2025gaspacho}, leverage synchronized camera arrays to disentangle human and object motions. 
While effective, these methods depend on complex capture setups that are impractical for in-the-wild applications. 
In contrast, HOIGS targets the more challenging monocular setting. We explicitly model the mutual influence between humans and objects, ensuring stable reconstruction and physically plausible interaction without requiring multi-view constraints.

\subsection{Dynamic Scene Representations}
\noindent\textbf{From Implicit Fields to 4D Gaussians.}
Dynamic scene modeling has shifted from implicit neural representations \cite{park2021nerfies, park2021hypernerf, wu2022d, fridovich2023k} to explicit temporal representations for improved efficiency. 
While NeRF-based dynamic methods achieved high visual quality, they are fundamentally limited by slow training and rendering times. 
To overcome this, 4D Gaussian Splatting (4DGS) methods \cite{wu20244d, yang2023real} extend the explicit Gaussian representation to the temporal domain. 
However, current 4DGS approaches face two critical limitations when applied to interaction-rich scenes. 
First, they typically rely on Structure-from-Motion (SfM) point clouds for initialization. 
Since SfM assumes a static world, it fails to generate accurate geometry for moving objects, leading to poor initialization for dynamic elements. 
Second, these methods often employ unified MLP-based deformation fields to model all scene dynamics. 
While sufficient for simple trajectories, implicit fields tend to over-smooth complex, high-frequency motions characteristic of manipulated objects. 
To address these gaps, we propose an explicit, spline-based motion model that disentangles object dynamics from human articulation, enabling high-fidelity rendering of complex temporal movements.

==> tex_main/2_Relatedwork.tex <==
\section{Related Works}

\subsection{3D Human Modeling}
% \noindent\textbf{Human Modeling.}
Research on realistic human modeling has long been pursued. Early parametric models enabled efficient estimation of human pose, exemplified by HMR (\textcolor{blue}{\cite{kanazawa2018end}}), but struggled to capture clothing and accessories. To address this, implicit function-based methods (\textcolor{blue}{\cite{huang2020arch, saito2019pifu, saito2020pifuhd, xiu2022icon, xiu2023econ}}) were proposed, which recover fine details such as hair and clothing but remain limited in global consistency and rendering efficiency. These methods mainly focused on human geometry with little attention to human-object interactions. With Neural Radiance Fields (NeRF) (\textcolor{blue}{\cite{mildenhall2021nerf}}), several works applied it to human modeling (\textcolor{blue}{\cite{peng2021neural, jiang2022neuman, weng2022humannerf, alldieck2022photorealistic, liao2023high, guo2023vid2avatar}}), achieving realistic appearance and view consistency but still suffering from high training cost and slow rendering. In terms of human-object interactions, some attempts (\textcolor{blue}{\cite{fan2024hold}}) introduced objects, yet dynamic interactions were not fully captured. Recently, 3D Gaussian Splatting (3DGS) (\textcolor{blue}{\cite{kerbl20233d}}) emerged as a new representation and has been applied to human reconstruction (\textcolor{blue}{\cite{kocabas2024hugs, moon2024expressive, hu2024gauhuman, liu2024animatable, hu2024gaussianavatar}}). However, most efforts still regard objects as static. 
Recent approaches leverage multi-view data for high-fidelity results. For example, Animatable Gaussian \cite{li2024animatable} and GASPACHO \cite{mir2025gaspacho} utilize multi-view setups to create relightable avatars and disentangle human-object interactions. However, these methods depend on complex capture settings, whereas real-world scenarios are predominantly monocular. To address this, we propose HOIGS, a model for stable human reconstruction that explicitly captures human–object interactions from monocular inputs.


 
\subsection{Dynamic Scene Modeling}
% \noindent\textbf{Dynamic Scene Modeling.}
The field of dynamic scene rendering and reconstruction has seen a paradigm shift from initial NeRF-based methods  (\textcolor{blue}{\cite{park2021nerfies, park2021hypernerf, wu2022d, fridovich2023k}}) to the more recent 3D Gaussian Splatting framework. Previous studies such as HOSNeRF (\textcolor{blue}{\cite{liu2023hosnerf}}) effectively modeled human-object interactions by controlling human motion through skeleton-based models such as SMPL and leveraging object state embeddings. Nevertheless, the implicit representation inherent to NeRF led to significant computational overhead in training and rendering, and limited the ability to represent detailed features in large-scale environments. To address this efficiency bottleneck, a line of work has emerged that extends 3DGS to the temporal domain, known as 4D Gaussian Splatting (4DGS) (\textcolor{blue}{\cite{wu20244d, yang2023real}}). Although these methods achieve real-time rendering speeds, they face persistent issues. Most 4DGS approaches rely on Structure-from-Motion for Gaussian initialization, which is fundamentally ill-suited for dynamic subjects as it operates on the assumption of a static world. This leads to inaccurate point cloud generation for moving objects. Moreover, the MLP-based implicit deformation fields used to capture motion, while adequate for simple trajectories, often result in over-smoothed or unnatural movements when applied to complex, in-the-wild scenarios. Therefore, we propose an explicit, spline-based motion model. This approach allows us to model intricate temporal movements with high fidelity, achieving high-quality rendering even in dynamic scenes that include complex human-object interactions.


==> tex_main/4_Method.tex <==
\input{tex_FIG/Method_main_fig}

\section{Method}
 
As shown in Fig. \textcolor{blue}{~\ref{figure_main_method}}, we reconstruct the scene by independently modeling the deformations of humans and objects, and then incorporating interaction-aware transformations through the HOI module. Object deformations are estimated using a Cubic Hermite Spline (CHS). Human deformations are based on HexPlane features, where time-invariant spatial features are used to learn the texture of the canonical T-pose, and Linear Blend Skinning (LBS) is subsequently applied to deform the canonical representation into each world space. Using these deformation baselines, we independently model humans and objects and estimate their approximate positions for each frame, from which motion features are extracted. Finally, the extracted human and object features are fed into the HOI module, which accounts for interaction-driven transformations and determines the final positions of humans and objects in the reconstructed interaction scene.
\subsection{Object deformation}
\subsubsection{Object Initialization.}
We begin by segmenting the object of interest and cropping the object region from a representative frame of the entire sequence. Next, we apply a diffusion model initialized from DreamScene4D~\cite{dreamscene4d} and guided by SDS loss to generate a canonical 3D Gaussian point cloud of the object. However, the 3D Gaussians generated through this diffusion prior may differ from the actual object geometry. While diffusion models can generate plausible 3D shapes from images, they often fail to precisely recover the true object structure. To address this, we align the diffusion-based canonical 3D Gaussians with the world space. First, we estimate a per-frame warping scale $S_t$ by minimizing the discrepancy between the projected 3D bounding box and the 2D mask bounding box for each frame $t$.
We then compute the global scale $S$ as the average over all frames:

\[
S_t = \arg\min_{S_t} \left\| \text{BBox}_{\text{proj}}(S_t \cdot \text{Gaussians}) - \text{BBox}_{\text{mask}}^t \right\|, \quad
S = \frac{1}{T} \sum_{t=1}^{T} S_t .
\]

where $T$ is the total number of frames. We then transform the scaled Gaussians to the world coordinate system using the COLMAP camera extrinsics $R_t$ and $\mathbf{t}_t$ as follows:

\[
\mathbf{x}_{\text{world}}^t = R_t^{-1} (\mathbf{x}_{\text{cam}}^t - \mathbf{t}_t).
\]

From the warped Gaussians $G_k$ of each keyframe, we extract each Gaussian’s mean and color value, while initializing the remaining 3D Gaussian parameters with identity values.

\subsubsection{Object Deformation.}
Based on the redefined mean and color from the keyframes, we construct the object’s 3D Gaussians and use them to model the object deformation. To represent the continuous motion of the object over time, we model the mean values of each Gaussian as control-point-based curves. Specifically, we define a Cubic Hermite Spline function $\text{CHS}(t, \mathbf{m})$, and estimate the position of an object Gaussian at time $t$, denoted as $\mathbf{M}(t)$, as follows:

\noindent This initialization ensures that the explicit 3D Gaussian deformation model aligns with the actual object geometry and structural information. 
From the warped Gaussians of each keyframe, we extract each Gaussian’s mean and color value, while initializing the remaining 3D Gaussian parameters with identity values.
We apply a diffusion prior with SDS loss to reconstruct the object from a representative frame of the entire sequence. The reconstructed object is then warped using the camera parameters of each keyframe to initialize the corresponding 3D Gaussians.
However, the 3D Gaussians generated through the diffusion prior may differ from the actual object geometry. While diffusion models can generate plausible 3D shapes from images, they often fail to precisely recover the true object structure. To address this, we introduce an explicit 3D Gaussian deformation model that aligns the diffusion-based initialization with the actual object geometry and structural information.
From the warped Gaussians $G_k$ of each keyframe, we extract each Gaussian's mean and color value, while initializing the remaining 3D Gaussian parameters with identity values. Based on the redefined mean and color from the keyframes, we construct the object’s 3D Gaussians and use them to model the object deformation.
To represent the continuous motion of the object over time, we model the mean values of each Gaussian as control-point-based curves. Specifically, we define a Cubic Hermite Spline function $CHS(t, \mathbf{m})$, and estimate the position of an object Gaussian at time $t$, denoted as $M(t)$, as follows:
\[
M(t) = CHS(t, \bold{m}),
\]
where $\bold{m} = \left\{ m_k \mid m_k \in \mathbb{R}^3 \right\}_{k \in [0, N_{key} - 1]}$ is a learnable set of control points representing the mean positions of the Gaussians at each key frame, and $N_{key}$ denotes the number of key frames. $CHS(t, \mathbf{m})$ is formulated as

\vspace{-2mm}

\begin{equation}
\begin{aligned}
CHS(t, \mathbf{m}) &= (2t_r^3 - 3t_r^2 + 1)m_{\lfloor  t_s  \rfloor} + (t_r^3 - 2t_r^2 + t_r)\tau_{\lfloor t_s \rfloor  } \\
&\quad + (-2t_r^3 + 3t_r^2)m_{\lfloor t_s  \rfloor + 1} + (t_r^3 - t_r^2)\tau_{\lfloor t_s \rfloor  + 1}, 
\end{aligned}
\end{equation}

where $t_r = t_s - \lfloor t_s  \rfloor $, $t_s = t_n (N_{key} - 1)$, $t_n = \frac{t}{N_f - 1}$ and $N_f$ denotes the number of all frames.
$m_{\lfloor t_s \rfloor}$ denotes the mean of the 3D Gaussians corresponding to the $\lfloor t_s \rfloor$-th key frame.

In the standard formulation, $\tau_{\lfloor t_s \rfloor}$ represents the tangent vector with respect to the means of the surrounding Gaussians, which is typically approximated as $\tau_{\lfloor t_s \rfloor} = \tfrac{1}{2}\left(m_{\lfloor t_s \rfloor+1} - m_{\lfloor t_s \rfloor-1}\right)$. Instead of using this fixed approximation, we reinterpret $\tau_{\lfloor t_s \rfloor}$ as a \textit{velocity vector} and employ it as a learnable parameter. By embedding this velocity, we construct motion features that better capture the dynamic behavior of objects over time.

The position parameter $\bold{m}$ between key frames is estimated via spline interpolation using both the Gaussian positions $m_k$ at the key frames and the corresponding velocity vectors $\tau_{ \lfloor k \rfloor }$. Only the Gaussians at the key frames are directly optimized during training. Once the intermediate Gaussians are estimated and rendered, the resulting gradients from the loss function are backpropagated to update the parameters of the corresponding key frame Gaussians.
Among the Gaussian parameters, rotation and opacity are defined as time-dependent variables. The rotation parameter is modeled using Spherical Linear Interpolation based on the Gaussian rotations at each key frame, enabling smooth transitions over time. The opacity parameter varies with time to account for occluded regions caused by object motion. In contrast, the scale parameter is kept constant across all corresponding Gaussians at different key frames.
\subsection{Human deformation}
\subsubsection{HexPlane-based Deformation.}
We model human deformation using HexPlane features. 
Specifically, we adopt time-invariant spatial features $f$ from HexPlane to learn the texture of the canonical T-pose mesh $T_c$ in the canonical space. The features $f$ are processed by an MLP head $\psi$ to learn the Gaussian properties in the canonical space. This representation serves as the baseline for human deformation. The canonical human representation is then deformed into the posed world space using Linear Blend Skinning (LBS) as follows:
\begin{equation}
\psi_h(f(T_c)) = (c, o, \Delta P_c, R, S, W),
\end{equation}
\begin{equation}
P_{def} = \alpha * LBS(P_c , \theta, W),
\end{equation}
where $\theta$ denotes the set of SMPL-X pose parameters and $\alpha$ is a learnable scale parameter for human pose. 
Equation (3) extracts the Gaussian properties (color $c$, opacity $o$, position offset $\Delta P_c$, rotation $R$, scale $S$ and skinning weights $W$) from the canonical HexPlane features, 
while Equation (4) applies the LBS function to obtain the deformed positions $P_{def}$ of the Gaussians in the posed space. 

To ensure that the reconstructed human representation matches the actual geometry, 
we further apply a depth supervision loss:
\begin{equation}
\mathcal{L}_{depth} = \left\| D_{render} - D \right\|_1,
\end{equation}
where $D_{render}$ is the rendered depth map from the deformed Gaussians and $D$ is the depth obtained from an off-the-shelf metric depth estimation model and further scaled using the COLMAP point cloud. 
This depth-guided supervision constrains the learnable scale parameter $\alpha$ and improves geometric fidelity in the reconstructed human shape.



\subsection{Cross-Attention Interaction Module}
\subsubsection{Feature Extraction.} We extract time-varying features from both humans and objects to learn their interactions. For humans, instead of relying on time-invariant texture features from the canonical space, we utilize time-varying features from HexPlane. Furthermore, since it is not possible to know in advance which body parts are involved in object interactions, we divide the human body into 16 parts and extract HexPlane features for each part.

For objects, the features are derived from the velocity embeddings associated with each keyframe in the deformation process, which capture the local motion information at those frames. In addition, we embed learnable parameters for each keyframe to represent latent motion characteristics that cannot be fully captured by velocity alone. These velocity vectors and learnable parameters are then projected together with the corresponding time values, enabling the construction of object motion features. This formulation allows us to obtain continuous motion features for objects across all frames, rather than being limited to discrete keyframes.

\subsubsection{Interaction Module.} The proposed Interaction module (HOI module) takes time-varying features of humans and objects as inputs and explicitly models their interactions. 
Let the human and object features be denoted as $F_{\text{Human}}$ and $F_{\text{Object}}$. 
To capture interdependencies between the two, we apply \textit{mutual attention}, where queries, keys, and values are defined as:
\begin{equation}
\begin{aligned}
Q_h, K_h, V_h &= F_{\text{Human}}W_h^Q,\; F_{\text{Human}}W_h^K,\; F_{\text{Human}}W_h^V, \\
Q_o, K_o, V_o &= F_{\text{Object}}W_o^Q,\; F_{\text{Object}}W_o^K,\; F_{\text{Object}}W_o^V.
\end{aligned}
\end{equation}
Cross-attention is then performed in both directions, from human to object and from object to human, while incorporating a distance mask $B$ into the attention computation:
\begin{equation}
F'_{\text{Human}} = \text{softmax}\!\left(\tfrac{Q_hK_o^\top}{\sqrt{d}} + B\right)V_h,\quad
F'_{\text{Object}} = \text{softmax}\!\left(\tfrac{Q_oK_h^\top}{\sqrt{d}} + B^\top\right)V_o.
\end{equation}




The distance mask $B$ filters out distant objects based on their 3D spatial proximity to the human.
Specifically, for each object, we compute the Euclidean distance between the object's Gaussian center $c_{\mathrm{obj}}^{\mathrm{world}}$ and the human pelvis position $p_{\mathrm{pelvis}}^{\mathrm{world}}$ in world coordinates. 
$B_{ij}$ encodes the relative distance between the $i$-th human token and the $j$-th object token:

\begin{equation}
B_{ij} = \begin{cases}
-\infty & \text{if } \lVert c_{\mathrm{obj}}^{\mathrm{world}} - p_{\mathrm{pelvis}}^{\mathrm{world}} \rVert \ge \tau \\
0 & \text{otherwise}
\end{cases},
\end{equation}
 
where $\tau$ is set to the human arm length (derived from the SMPL-X model). When $B_{ij}=-\infty$, the corresponding object tokens are masked out during attention, effectively excluding non-interacting background objects.

This process yields updated features $F'_{\text{Human}}$ and $F'_{\text{Object}}$ that embed interaction cues. 
Finally, $F'_{\text{Human}}$ is used to regress $\Delta$SMPL-X refinements (body pose, hand pose), while $F'_{\text{Object}}$ is used to predict $\Delta G_{\text{object}}$, i.e., corrections for Gaussian-based object motion. 
In this way, the HOI module augments the baseline deformations (HexPlane+LBS for humans and CHS for objects) with interaction-aware adjustments, enabling accurate reconstruction of human--object interaction scenes.


\subsection{Optimization} For background modeling, we employ the standard 3D Gaussian Splatting (3DGS) technique. During training, we isolate the background by masking out the object and human regions, allowing the static Gaussian background to be optimized using a photometric loss. For human modeling, we regress the SMPL-X parameters by \cite{moon2022accurate}, and incorporate an SMPL-X-based avatar model to ensure natural interaction with the object. For each frame, we extract the SMPL-X parameters and define a canonical T-pose human avatar. This canonical avatar is then deformed to match each frame using LBS. During training, image-based loss metrics such as SSIM, LPIPS, and L1-norm were utilized to compare the Gaussian renderer's output with the human region in the image. 

\subsubsection{Object Motion Optimization.} We model the motion of objects using CHS to ensure continuity in position interpolation. A CHS is a piecewise cubic polynomial that is defined by both the positions and the first derivatives (tangents) at key points in time. By specifying the starting and ending slopes for each spline segment, CHS guarantees smooth transitions between key frames, maintaining continuity not only in the object’s position but also in its velocity. In other words, the object’s trajectory over time remains continuous and smooth, without abrupt jumps or changes in speed. This property is crucial for accurately modeling temporal motion in a realistic and stable manner.

\subsubsection{Integrated Optimization.} We train our model using an integrated optimization objective that combines multiple loss terms. Specifically, the overall loss function is formulated as:
\[
\mathcal{L} = \gamma \, \mathcal{L}_{\text{object motion}} + \beta \, \mathcal{L}_{\text{human}} + \sigma \, \mathcal{L}_{\text{scene}} + \mathcal{L}_{\text{depth}},
\]
where $\mathcal{L}_{\text{object motion}}$, $\mathcal{L}_{\text{human}}$, and $\mathcal{L}_{\text{scene}}$ are the loss components for the object's motion, the human-related factors, and the scene context, respectively. Here, $\gamma$, $\beta$, and $\sigma$ are hyperparameters that control the relative weight of each loss term during training. By tuning these hyperparameters, we balance the influence of each component on the training objective. This integrated optimization approach ensures that the model simultaneously accounts for object motion accuracy, human interaction plausibility, and scene consistency during learning.


==> tex_main/4_Method_HOI.tex <==

\subsection{Cross-Attention Interaction Module}
\label{sec:hoi_module}

To address the limitations of independent modeling, we propose an Interaction (HOI) module that explicitly learns the interdependencies between human and object motions.

\textbf{Object feature}.
%우리는 object feature를 추출하기 위해 key frame의 Gaussian에 대해 velocity vector와 임베딩 파라미터를 활용한다. 각 key frame의 velocity vector는 CHS에 적용되어 baseline deformation과 함께 HOI module의 입력 feature로 공동 최적화된다. 추가적으로 각 key frame의 Gaussian마다 29차원의 learnable parameter를 임베딩하며, 이 임베딩은 velocity vector와 결합되어 feature로 사용된다. CHS를 통해 interpolation된 Gaussian feature는 결합된 feature와 time 정보를 입력으로 받아 얕은 MLP layer를 거쳐 projection되며, 최종적으로 32차원의 feature를 형성한다.
As shown in Fig. \textcolor{blue}{\ref{appendix_objfeature}}(a), we extract object features by leveraging the velocity vectors and embedding parameters of Gaussians at key frames. As shown in Fig. \textcolor{blue}{\ref{appendix_objfeature}}(b), each key frame’s velocity vector is applied to the CHS and jointly optimized with the baseline deformation as input features for the HOI module. In addition, a 29-dimensional learnable parameter is embedded for each key frame Gaussian, which is concatenated with the velocity vector to form the feature representation. The interpolated Gaussian features produced by CHS are then combined with the concatenated feature and time information, and projected through a shallow MLP, resulting in a 32-dimensional feature vector.


\textbf{Human feature}.
Fig. \textcolor{blue}{~\ref{appendix_humanfeature}} illustrates the process of human feature extraction. 
We divide the SMPL-X model into 16 body parts and learn features corresponding to each part. 
Temporal features are sampled from the HexPlane at SMPL-X vertices, where each feature at time $t$ is obtained based on the coordinates $(x_t, y_t, z_t)$. 
For each body part, the features of its associated vertices are averaged to form the part-specific representation $F_{\text{human}}$: 
\[
F_{\text{part}} = \frac{1}{N} \sum_{i \in \text{part}} f_i(x_t, y_t, z_t),
\]
where $N$ denotes the number of vertices belonging to the part. 
As a result, 16 part features, including head, torso, arms, and legs, are obtained and used as inputs to the HOI module. 
This design captures temporally varying dynamic representations while preserving semantically meaningful features for individual body parts.

% \subsubsection{Feature Extraction.}
% We extract time-varying features for both entities. For the human, we partition the body into 16 semantic parts and extract time-dependent HexPlane features $F_{\text{Human}}$ for each part. 
% For the object, we construct motion features $F_{\text{Object}}$ by projecting the learnable velocity vectors $\boldsymbol{\tau}$ and latent motion codes associated with each keyframe. This projection incorporates temporal embeddings, providing continuous motion contexts $F_{\text{Object}}$ across all frames.


\subsubsection{Interaction Module.}
We capture the bidirectional influence between human and object features using a mutual attention mechanism. The features are projected into queries ($Q$), keys ($K$), and values ($V$) via linear layers (\textit{e.g.}, $Q_h = F_{\text{Human}}W_h^Q$). We compute the updated features with a spatial distance mask $B$:
\begin{equation}
F'_{\text{Human}} = \text{softmax}\!\left(\frac{Q_h K_o^\top}{\sqrt{d}} + B\right)V_h, \quad
F'_{\text{Object}} = \text{softmax}\!\left(\frac{Q_o K_h^\top}{\sqrt{d}} + B^\top\right)V_o.
\end{equation}
The mask $B_{ij}$ filters out non-interacting object tokens based on the Euclidean distance between the object center $c_{\mathrm{obj}}^{\mathrm{world}}$ and the human pelvis $p_{\mathrm{pelvis}}^{\mathrm{world}}$.
If the distance exceeds a threshold $\tau$ (set to the arm length derived from SMPL-X), $B_{ij} = -\infty$, effectively masking the interaction.
The updated features $F'_{\text{Human}}$ and $F'_{\text{Object}}$ are then used to regress refinements for the SMPL-X parameters (body/hand pose corrections) and object Gaussian trajectories ($\Delta G_{\text{object}}$), respectively.

\subsection{Optimization}
\label{sec:optimization}

We employ an integrated optimization strategy that jointly refines the background, human, and object representations.
The static background is modeled using standard 3D Gaussian Splatting (3DGS) and optimized via photometric loss, masking out dynamic regions.
For human modeling, we initialize SMPL-X parameters using the method of Moon et al.~\cite{moon2022accurate} and define a canonical avatar deformed via LBS. Standard image-based losses (L1, SSIM, LPIPS) are applied to the rendered human regions.

The total loss function combines terms for object motion, human fidelity, and scene consistency:
\begin{equation}
\mathcal{L} = \gamma \, \mathcal{L}_{\text{object}} + \beta \, \mathcal{L}_{\text{human}} + \sigma \, \mathcal{L}_{\text{scene}} + \mathcal{L}_{\text{depth}},
\end{equation}
where $\mathcal{L}_{\text{object}}$ enforces smoothness and accuracy in the spline-based trajectory, and $\mathcal{L}_{\text{human}}$ ensures the plausibility of the human pose and shape. The hyperparameters $\gamma$, $\beta$, and $\sigma$ balance the contribution of each component.
This unified objective ensures that the model simultaneously recovers accurate object trajectories, plausible human deformations, and consistent interactions.






Specifically, the canonical T-pose mesh $T_c$ is partitioned into 16 semantic parts, denoted by a set $\mathcal{P} = \{ \text{head}, \text{torso}, \text{left\_arm}, \text{left\_hand}, \dots \}$. For each part $p \in \mathcal{P}$, we compute the part-level feature $F_p$ by average pooling the queried features:

\begin{equation}
F_p = \frac{1}{N_p} \sum_{i \in p} f(x_i, y_i, z_i), \label{eq:part_feature}
\end{equation}

where $N_p$ denotes the number of vertices belonging to part $p$, and $(x_i, y_i, z_i)$ are the canonical coordinates. Consequently, the holistic human representation $F_{\text{human}}$ is formulated as a collection of these semantic part features:

\begin{equation}
F_{\text{human}} = \big\{ F_{\text{head}}, F_{\text{torso}}, F_{\text{left\_arm}}, F_{\text{left\_hand}}, \dots \big\} = \{ F_p \mid p \in \mathcal{P} \}, \label{eq:human_feature}
\end{equation}

which serves as the comprehensive input for the subsequent HOI module.

==> tex_main/4_Method_revised_2.tex <==
\input{tex_FIG/Method_main_fig}

\section{Method}
 
As shown in Fig. \textcolor{blue}{~\ref{figure_main_method}}, we reconstruct the scene by independently modeling the deformations of humans and objects, and then incorporating interaction-aware transformations through the HOI module. Object deformations are estimated using a Cubic Hermite Spline (CHS)~\cite{deboor1978practical}. Human deformations are based on HexPlane features~\cite{cao2023hexplane, fridovich2023kplanes}, where time-invariant spatial features are used to learn the texture of the canonical T-pose, and Linear Blend Skinning (LBS)~\cite{magnenat1988joint} is subsequently applied to deform the canonical representation into each world space. Using these deformation baselines, we independently model humans and objects and estimate their approximate positions for each frame, from which motion features are extracted. Finally, the extracted human and object features are fed into the HOI module, which accounts for interaction-driven transformations and determines the final positions of humans and objects in the reconstructed interaction scene.

\subsection{Object deformation}
\subsubsection{Object Initialization.}
We begin by segmenting the object of interest and cropping the object region from a representative frame of the entire sequence. Next, we apply a diffusion model initialized from DreamScene4D~\cite{dreamscene4d} and guided by SDS loss~\cite{poole2022dreamfusion} to generate a canonical 3D Gaussian point cloud of the object. However, the 3D Gaussians generated through this diffusion prior may differ from the actual object geometry. While diffusion models can generate plausible 3D shapes from images, they often fail to precisely recover the true object structure. To address this, we align the diffusion-based canonical 3D Gaussians with the world space. First, we estimate a per-frame warping scale $S_t$ by minimizing the discrepancy between the projected 3D bounding box and the 2D mask bounding box for each frame $t$. We then compute the global scale $S$ as the average over all frames:

\[
S_t = \arg\min_{S_t} \left\| \text{BBox}_{\text{proj}}(S_t \cdot \text{Gaussians}) - \text{BBox}_{\text{mask}}^t \right\|, \quad
S = \frac{1}{T} \sum_{t=1}^{T} S_t .
\]

where $T$ is the total number of frames. We then transform the scaled Gaussians to the world coordinate system using the COLMAP~\cite{schonberger2016structure} camera extrinsics $R_t$ and $\mathbf{t}_t$ as follows:

\[
\mathbf{x}_{\text{world}}^t = R_t^{-1} (\mathbf{x}_{\text{cam}}^t - \mathbf{t}_t).
\]

From the warped Gaussians $G_k$ of each keyframe, we extract each Gaussian’s mean and color value, while initializing the remaining 3D Gaussian parameters with identity values.

\subsubsection{Object Deformation.}
Based on the redefined mean and color from the keyframes, we construct the object’s 3D Gaussians and use them to model the object deformation. To represent the continuous motion of the object over time, we model the mean values of each Gaussian as control-point-based curves. Specifically, we define a Cubic Hermite Spline function $\text{CHS}(t, \mathbf{m})$~\cite{ahlberg2016theory}, and estimate the position of an object Gaussian at time $t$, denoted as $\mathbf{M}(t)$, as follows:
\[
M(t) = CHS(t, \bold{m}),
\]
where $\bold{m} = \left\{ m_k \mid m_k \in \mathbb{R}^3 \right\}_{k \in [0, N_{key} - 1]}$ is a learnable set of control points representing the mean positions of the Gaussians at each key frame, and $N_{key}$ denotes the number of key frames. $CHS(t, \mathbf{m})$ is formulated as

\vspace{-2mm}

\begin{equation}
\begin{aligned}
CHS(t, \mathbf{m}) &= (2t_r^3 - 3t_r^2 + 1)m_{\lfloor  t_s  \rfloor} + (t_r^3 - 2t_r^2 + t_r)\tau_{\lfloor t_s \rfloor  } \\
&\quad + (-2t_r^3 + 3t_r^2)m_{\lfloor t_s  \rfloor + 1} + (t_r^3 - t_r^2)\tau_{\lfloor t_s \rfloor  + 1}, 
\end{aligned}
\end{equation}

where $t_r = t_s - \lfloor t_s  \rfloor $, $t_s = t_n (N_{key} - 1)$, $t_n = \frac{t}{N_f - 1}$ and $N_f$ denotes the number of all frames. $m_{\lfloor t_s \rfloor}$ denotes the mean of the 3D Gaussians corresponding to the $\lfloor t_s \rfloor$-th key frame. In the standard formulation, $\tau_{\lfloor t_s \rfloor}$ represents the tangent vector with respect to the means of the surrounding Gaussians, which is typically approximated as $\tau_{\lfloor t_s \rfloor} = \tfrac{1}{2}\left(m_{\lfloor t_s \rfloor+1} - m_{\lfloor t_s \rfloor-1}\right)$. Instead of using this fixed approximation, we reinterpret $\tau_{\lfloor t_s \rfloor}$ as a \textit{velocity vector} and employ it as a learnable parameter. By embedding this velocity, we construct motion features that better capture the dynamic behavior of objects over time. The position parameter $\bold{m}$ between key frames is estimated via spline interpolation using both the Gaussian positions $m_k$ at the key frames and the corresponding velocity vectors $\tau_{ \lfloor k \rfloor }$. Only the Gaussians at the key frames are directly optimized during training. Once the intermediate Gaussians are estimated and rendered, the resulting gradients from the loss function are backpropagated to update the parameters of the corresponding key frame Gaussians.

Among the Gaussian parameters, rotation and opacity are defined as time-dependent variables. The rotation parameter is modeled using Spherical Linear Interpolation based on the Gaussian rotations at each key frame, enabling smooth transitions over time. The opacity parameter varies with time to account for occluded regions caused by object motion. In contrast, the scale parameter is kept constant across all corresponding Gaussians at different key frames; while distribution-aware quantization methods~\cite{hong2022daq} suggest adaptive scaling for efficiency, we maintain constant scaling to ensure geometric consistency in dynamic interaction.

\subsection{Human deformation}
\subsubsection{HexPlane-based Deformation.}
We model human deformation using HexPlane features, inspired by recent advances in hybrid avatar representations~\cite{moon2024exavatar}. Specifically, we adopt time-invariant spatial features $f$ from HexPlane to learn the texture of the canonical T-pose mesh $T_c$ in the canonical space. The features $f$ are processed by an MLP head $\psi$ to learn the Gaussian properties in the canonical space. This representation serves as the baseline for human deformation. The canonical human representation is then deformed into the posed world space using Linear Blend Skinning (LBS)~\cite{magnenat1988joint} as follows:
\begin{equation}
\psi_h(f(T_c)) = (c, o, \Delta P_c, R, S, W),
\end{equation}
\begin{equation}
P_{def} = \alpha * LBS(P_c , \theta, W),
\end{equation}
where $\theta$ denotes the set of SMPL-X pose parameters~\cite{pavlakos2019expressive} and $\alpha$ is a learnable scale parameter for human pose. Equation (3) extracts the Gaussian properties (color $c$, opacity $o$, position offset $\Delta P_c$, rotation $R$, scale $S$ and skinning weights $W$) from the canonical HexPlane features, while Equation (4) applies the LBS function to obtain the deformed positions $P_{def}$ of the Gaussians in the posed space. To ensure that the reconstructed human representation matches the actual geometry, we further apply a depth supervision loss:
\begin{equation}
\mathcal{L}_{depth} = \left\| D_{render} - D \right\|_1,
\end{equation}
where $D_{render}$ is the rendered depth map... and the first derivatives (tangents) at key points in time. By specifying the starting and ending slopes for each spline segment, CHS guarantees smooth transitions between key frames, maintaining continuity not only in the object’s position but also in its velocity. In other words, the object’s trajectory over time remains continuous and smooth, without abrupt jumps or changes in speed. This property is crucial for accurately modeling temporal motion in a realistic and stable manner.

\subsubsection{Integrated Optimization.} We train our model using an integrated optimization objective that combines multiple loss terms. Specifically, the overall loss function is formulated as:
\[
\mathcal{L} = \gamma \, \mathcal{L}_{\text{object motion}} + \beta \, \mathcal{L}_{\text{human}} + \sigma \, \mathcal{L}_{\text{scene}} + \mathcal{L}_{\text{depth}},
\]
where $\mathcal{L}_{\text{object motion}}$, $\mathcal{L}_{\text{human}}$, and $\mathcal{L}_{\text{scene}}$ are the loss components for the object's motion, the human-related factors, and the scene context, respectively. Here, $\gamma$, $\beta$, and $\sigma$ are hyperparameters that control the relative weight of each loss term during training. By tuning these hyperparameters, we balance the influence of each component on the training objective, similar to strategies employed in task-adaptive learning~\cite{baik2021meta}. This integrated optimization approach ensures that the model simultaneously accounts for object motion accuracy, human interaction plausibility, and scene consistency during learning.

==> tex_main/5_Experiments.tex <==
\section{Experiments}

% \subsection{Implementation Details}
We use ExAvatar (\textcolor{blue}{\cite{moon2024expressive}}) as the baseline human rendering model, and all hyperparameters are kept identical to those used in ExAvatar. For object deformation using splines (\textcolor{blue}{\cite{ahlberg2016theory, de1978practical}}), we fix the time interval to 4 for all scenes. Training is conducted using an NVIDIA H100 GPU, taking approximately 5 hours per scene.
\vspace{-5pt}
\subsection{Datasets}
\subsubsection{HOSNeRF dataset \cite{liu2023hosnerf}.} We use the monocular dynamic-scene dataset HOSNeRF, which captures human–object interaction scenarios. The dataset comprises recordings in six indoor and outdoor locations with six subjects interacting with objects within a single scenario. Each sequence contains 300–400 frames. For evaluation, we uniformly select 16 frames per sequence for testing and use the remaining frames for training, following HOSNeRF.
\subsubsection{BEHAVE dataset{\cite{bhatnagar2022behave}}.} We use the BEHAVE multi-view RGB-D human–object interaction dataset, but adapt it to a monocular setting by selecting a single fixed camera from the four static viewpoints for each sequence. Specifically, we curate 9 sequences covering four distinct indoor environments, five subjects, and four objects. From each sequence’s raw video, we uniformly sample 300 frames. For evaluation, we uniformly select 16 frames per sequence for testing and use the remaining frames for training 
\subsubsection{}
\textbf{ARCTIC dataset (\textcolor{blue}{\cite{fan2023arctic}}).} We use the ARCTIC hand–object interaction dataset and extend comparisons to hand–object baselines. Since HOIGS is human-centric rather than hand-only, we evaluate only sequences where the full body is visible. Specifically, we use sequences of one subject interacting with four objects. Each monocular sequence (≈600 frames) is split by uniformly sampling 16 frames for testing and using the rest for training.


\input{tex_FIG/Experiments_hosnerf}
\input{tex_FIG/Experiments_behave}
\input{tex_FIG/Experiments_arctic}
\input{tex_Tables/HOSNeRF_dataset}
\input{tex_Tables/BEHAVE_dataset}
\input{tex_Tables/ARCTIC_dataset}

\subsection{Qualitative results}

We compare our view-synthesis results with existing Gaussian-based models, which generally outperform NeRF-based methods in rendering quality. The experimental results are visualized in Fig. ~\textcolor{blue}{\ref{fig:visual_HOSNeRF}}. The dynamic-scene models D3DGS (\textcolor{blue}{\cite{yang2024deformable}}) and Ex4DGS (\textcolor{blue}{\cite{lee2024fully}}) yield ghosting artifacts for both human and dynamic objects because they fail to disentangle human and object motions within complex interactions. ExAvatar (\textcolor{blue}{\cite{moon2024expressive}}) reconstructs humans but does not handle dynamic objects. Our method accurately reconstructs humans and objects with temporally coherent motion, using CHS object trajectories with velocity vectors and the human backbone based on HexPlane and LBS, while the HOI module further ensures contact consistency. On the ARCTIC dataset, as shown in Fig.~\textcolor{blue}{\ref{fig:visual_ARCTIC}}, HOLD (\textcolor{blue}{\cite{fan2024hold}}) shows limited performance in full-body–object interactions, whereas HOIGS successfully reconstructs them. This is because HOLD reconstructs only hands, while HOIGS reconstructs the entire human body including the hands. On the BEHAVE dataset, as shown in Fig.~\textcolor{blue}{\ref{fig:visual_BEHAVE}}, whereas ExAvatar suffers body–background overlap due to human misalignment in world space, our depth-based alignment ensures accurate human placement. Through qualitative results, we further confirm that our method effectively reconstructs complex human–object interactions with visually consistent outcomes.


\subsection{Quantitative results}
As shown in Tab.~\textcolor{blue}{\ref{tab:hosnerf_comparison}}, HOIGS achieves the highest PSNR and the lowest LPIPS on the Backpack, Tennis, Suitcase, Dance, and Lounge scenarios of the HOSNeRF dataset, surpassing prior 3D Gaussian-based models in visual quality. Tab.~\textcolor{blue}{\ref{tab:BEHAVE_comparison}} shows that on the BEHAVE dataset, it likewise attains the highest PSNR and lowest LPIPS, demonstrating effective reconstruction of complex human–object interactions from single-view input. Tab.~\textcolor{blue}{\ref{tab:ARCTIC_comparison}} shows that on the ARCTIC dataset, our method outperforms the hand–object model HOLD  (\textcolor{blue}{\cite{fan2024hold}}). Unlike HOLD, our model reconstructs complex full-body geometry while simultaneously capturing interactions with dynamic objects. 



\subsection{Ablation study}

\input{tex_Tables/ablation}
We conduct ablation studies to validate the effectiveness of the proposed method. As shown in Tab.~\textcolor{blue}{\ref{ablation}}, modeling object deformation with a simple MLP yields the lowest performance, while our CHS-based baseline deformation improves PSNR by 0.5, demonstrating its superiority. Removing the HOI module and applying only velocity further results in a 0.6 drop in PSNR compared to the full model, confirming the necessity of explicitly modeling human–object interactions. Finally, replacing the time-varying HexPlane features with simple parameter embeddings for the human features leads to a 0.2 decrease in PSNR, highlighting the effectiveness of our human feature design.

==> tex_main/6_Conclusion.tex <==
\section{Conclusion}
We presented HOIGS, a novel framework for reconstructing dynamic scenes with explicit modeling of human–object interactions from monocular videos. By combining HexPlane-based~\cite{cao2023hexplane} human deformation, spline-based object motion, and an interaction-aware HOI module, our method achieves stable and accurate reconstruction even in challenging scenarios with contact and manipulation. In particular, the explicit treatment of human-object interactions enables our framework not only to recover realistic human geometry but also to faithfully capture object dynamics and their mutual influences, which have been largely overlooked in prior works. Extensive experiments on HOSNeRF, BEHAVE, and ARCTIC datasets demonstrate that HOIGS outperforms state-of-the-art human-centric and 4D Gaussian approaches in both visual quality and consistency, highlighting its effectiveness in advancing realistic modeling of complex human–object interactions.

\textbf{Limitations.}

\textbf{Future works.}
% \textbf{Limitations and future works.} While our framework handles typical dynamic motions well, it struggles under minimal camera movement, where COLMAP-based pose and point cloud estimation becomes unreliable. This often leads to rendering artifacts. Future work may improve robustness in such low-baseline settings by jointly optimizing camera poses during training.


% 사람에 대해서 novel pose가 주어질 경우, 새로운 장면을 만들 수 있다. 다만, 객체에 대해서는 사람에 종속적으로 영향을 받는 연구가



==> tex_main/6_Conclusion_revised.tex <==
\section{Conclusion}

We presented HOIGS, a novel framework for reconstructing dynamic scenes with explicit modeling of human--object interactions from monocular videos. By combining HexPlane-based human deformation, spline-based object motion, and an interaction-aware HOI module, our method achieves stable and accurate reconstruction even in challenging scenarios with contact and manipulation. In particular, the explicit treatment of human--object interactions enables our framework not only to recover realistic human geometry but also to faithfully capture object dynamics and their mutual influences, which have been largely overlooked in prior works. Extensive experiments on HOSNeRF, BEHAVE, and ARCTIC datasets demonstrate that HOIGS outperforms state-of-the-art human-centric and 4D Gaussian approaches in both visual quality and consistency, highlighting its effectiveness in advancing realistic modeling of complex human--object interactions.

\paragraph{Limitations.} 
Despite the high-fidelity reconstruction capabilities of HOIGS, our framework has limitations regarding object deformability. As described in Sec.~3.1, our method assumes object rigidity by keeping scale parameters constant across keyframes to stabilize the Cubic Hermite Spline optimization. Consequently, the model may struggle to accurately reconstruct highly deformable objects (\textit{e.g.}, soft tissues, fabrics, or fluids) that undergo significant topological changes or compression during interactions. Additionally, our pipeline relies on off-the-shelf diffusion models for the initial 3D object geometry and pre-computed SMPL-X parameters; therefore, severe inaccuracies in these initializations can propagate to the final reconstruction, particularly in cases of extreme occlusion where upstream estimators fail.

\paragraph{Future Work.} 
Future research will focus on relaxing the rigidity constraints to handle non-rigid object interactions. Integrating physics-based priors—such as collision handling and soft-body dynamics—into the Gaussian Splatting optimization process could enable more realistic deformations for soft objects. Furthermore, we aim to reduce the dependency on fixed pre-processing by jointly refining the human pose estimation and object initialization within the 3DGS optimization loop, allowing for a fully end-to-end reconstruction pipeline that is robust to initialization noise.

==> tex_main/6_Conclusion_revised_3.tex <==
\section{Conclusion}

We have presented HOIGS, a novel framework for reconstructing dynamic human--object interaction scenes from monocular RGB videos. Our method achieves high-fidelity reconstruction by explicitly modeling the interplay between human motion and object dynamics through three key innovations: HexPlane-based human deformation, spline-based object motion, and an interaction-aware HOI module. By explicitly treating human--object interactions as a first-class modeling primitive, HOIGS enables accurate recovery of both human geometry and object dynamics while preserving their mutual dependencies---capabilities that have been largely overlooked in prior work.

Extensive experiments on HOSNeRF, BEHAVE, and ARCTIC datasets demonstrate that HOIGS outperforms state-of-the-art human-centric and 4D Gaussian methods in both visual quality and temporal consistency. The superior performance validates the effectiveness of our design choices, particularly the explicit modeling of contact and manipulation dynamics. Our work represents a significant step toward realistic reconstruction of complex human--object interactions, opening new possibilities for applications in virtual reality, robotics, and human motion analysis.

\paragraph{Limitations.} 
Despite achieving high-fidelity reconstruction, our method has inherent constraints that suggest directions for future research. First, HOIGS assumes object rigidity by maintaining constant scale parameters across keyframes during Cubic Hermite Spline optimization. While this design choice ensures optimization stability, it limits our ability to reconstruct highly deformable objects such as cloth, soft tissues, or fluids that undergo significant topological changes during interaction. Second, our pipeline relies on external models for initial 3D object shape extraction and SMPL-X parameter estimation. Consequently, inaccurate initialization caused by factors such as severe occlusion or complex hand-object configurations can lead to error propagation in the final reconstruction. These dependencies highlight the need for more robust initialization strategies or end-to-end learning approaches.

\paragraph{Future Directions.} 
We identify three promising research directions to address current limitations and extend our framework's capabilities. \textit{First}, integrating physics-aware constraints into the 3DGS optimization process would enable more realistic deformations. Specifically, incorporating collision handling and contact dynamics between humans and objects could improve reconstruction quality while maintaining physical plausibility. \textit{Second}, developing a fully end-to-end pipeline that jointly refines human pose estimation and object initialization within the Gaussian Splatting optimization loop would reduce dependency on fixed preprocessing steps and improve robustness to initialization noise. \textit{Third}, while our current approach supports novel view synthesis given new human poses, modeling object dynamics that are causally influenced by human motion and interaction forces remains an open challenge. Addressing this would enable more comprehensive scene understanding and predictive capabilities, moving beyond reconstruction toward physics-based simulation of human--object interactions.

==> tex_main/7_Supplement_revised.tex <==

\begin{center}
\textbf{\large Supplementary Material \textit{for} \\ \vspace{2mm}
\large{"HOIGS: Human-Object Interaction Gaussian Splatting from Monocular Videos"}}
\end{center}

\setcounter{section}{0}
\setcounter{table}{0}
\setcounter{figure}{0}


\renewcommand{\thesection}{\Alph{section}}   
\renewcommand{\thetable}{\Alph{table}}   
\renewcommand{\thefigure}{\Alph{figure}}

In this supplementary material, we provide more experiments, discussions, and other details that could not be included in the main text due to the lack of pages.
The contents are summarized below.


% \input{src_suppl/co_registration_smplx}
% \input{src_suppl/mlp_architecture}
% \input{src_suppl/regularizers}
% \input{src_suppl/running_time_comparison}
% \input{src_suppl/geometry_comparison}
% \input{src_suppl/comparison_to_gen_ai}
% \input{src_suppl/implementation_details} 
% \input{src_suppl/failure_cases}


% \begin{compactitem}
%     \item Sec.~\ref{sec:co_registration_smplx}: Details of co-registration of SMPL-X
%     \item Sec.~\ref{sec:mlp_architecture}: Detailed architecture of MLPs
%     \item Sec.~\ref{sec:regularizers}: Regularizers
%     \item Sec.~\ref{sec:running_time_compare}: Running time comparison
%     \item Sec.~\ref{sec:geometry_comparison}: 3D geometry comparison
%     \item Sec.~\ref{sec:compare_to_gen_ai}: Comparison to generative AIs
%     \item Sec.~\ref{sec:implementation_details}: Implementation details
%     \item Sec.~\ref{sec:failure_cases}: Failure cases
% \end{compactitem}


\subsection{Quantitative Evaluation of Human Pose Accuracy}




{
\textbf{Geometric Fidelity Analysis}. 
We acknowledge that rendering metrics alone are insufficient to fully validate the geometric fidelity of complex human–object interactions. To address this, we conducted additional evaluations on human pose accuracy using the BEHAVE dataset. We compare our method against ExAvatar using PA-MPJPE (Procrustes Aligned Mean Per Joint Position Error) and PA-PVE (Procrustes-Aligned Per Vertex Error).
}



{
\textbf{Effect of the HOI Module on Pose Refinement}.
Our method explicitly models the mutual dependency between the human and the object. The HOI module leverages a cross-attention mechanism to use object motion features as contextual cues to refine human features. Specifically, as described in Eq. 14 of the main paper, the module predicts refinement offsets $\Delta$SMPL-X for the body and hands. This capability allows the network to correct the human pose—even under partial occlusion—by inferring the likely body configuration from the object's trajectory.
}



{
\textbf{Quantitative Results}.
Table \ref{tab:unified_comparison} summarizes the evaluation on the BEHAVE dataset. We report the average PA-MPJPE and PA-PVE across all test frames. Additionally, we provide a specific analysis for Hand and Forearm joints, which are the most critical regions for interaction tasks.
}
{
As shown in Table \ref{tab:unified_comparison}, HOIGS consistently outperforms the baseline. Notably, we observe a larger performance gain in the \textbf{PA-MPJPE (Hand/Forearm joints)}. This indicates that our HOI module effectively refines the poses of interaction-related body parts, resulting in physically more accurate reconstructions compared to ExAvatar, which lacks mutual feedback between the human and the object.}
\input{tex_Tables/Appendix_BEHAVE}

\subsection{Sensitivity Analysis on External Modules}

\input{tex_Tables/Appendix_External}  % COMMENTED OUT - file may be missing


{
\textbf{Robustness to External Priors.}~
To address concerns regarding the reliance on external modules, we conducted a sensitivity analysis on the HOSNeRF dataset by evaluating our framework with various combinations of segmentation (\textit{e.g.}, Samurai~\cite{yang2024samurai}, SAMv2~\cite{ravi2024sam2}, MaskRCNN~\cite{massa2018mrcnn}, TrackAnything~\cite{yang2023track}) and depth estimation (\textit{e.g.}, Video Depth Anything~\cite{video_depth_anything}, MetricV2~\cite{hu2024metric3dv2}, DepthCrafter~\cite{hu2025-DepthCrafter}) models.~
As shown in Table~\ref{tab:sensitivity_analysis}, HOIGS maintains highly consistent performance (Avg PSNR 25.8--26.1) across different modern priors, demonstrating that our method is robust to variations in preprocessing quality.~
Notably, even when employing the standard, older baseline of MaskRCNN combined with MetricV2, our model achieves an average PSNR of 25.44.~
This performance remains significantly higher than the state-of-the-art human-centric baseline, ExAvatar (Avg PSNR 24.35), and the 4DGS baseline, Ex4DGS (Avg PSNR 17.97).
}


% {
% \textbf{Robustness to External Priors.} 
% To address concerns regarding the reliance on external modules, we conducted a sensitivity analysis on the HOSNeRF dataset by evaluating our framework with various combinations of segmentation (\textit{e.g.}, Samurai, SAMv2, MaskRCNN, TrackAnything) and depth estimation (\textit{e.g.}, Video Depth Anything, MetricV2, DepthCrafter) models. 
% As shown in Table~\ref{tab:sensitivity_analysis}, HOIGS maintains highly consistent performance (Avg PSNR 25.8--26.1) across different modern priors, demonstrating that our method is robust to variations in preprocessing quality. 
% Notably, even when employing the standard, older baseline of MaskRCNN combined with MetricV2, our model achieves an average PSNR of 25.44. 
% This performance remains significantly higher than the state-of-the-art human-centric baseline, ExAvatar (Avg PSNR 24.35), and the 4DGS baseline, Ex4DGS (Avg PSNR 17.97).
% }

 
\subsection{Computational Complexity and Runtime Analysis}
{
\textbf{Runtime Performance}.
We evaluate the computational efficiency of our method on the HOSNeRF dataset using a single NVIDIA H100 GPU. As shown in Table~\ref{tab:runtime_comparison}, our method achieves an inference speed of \textbf{44.27 FPS}. While this is slightly lower than 4DGS~\cite{wu20244d} (61.04 FPS), it remains comparable to Ex4DGS~\cite{lee2024fully} (46.38 FPS) and outperforms D3DGS~\cite{yang2024deformable} (37.79 FPS). This result confirms that the inclusion of the HOI attention mechanism does not create a significant bottleneck, allowing our method to comfortably support real-time applications.
}
\input{tex_Tables/Appendix_Runtime}  % COMMENTED OUT - file may be missing

{
\textbf{Complexity Analysis}.
The efficiency of our HOI module stems from the token-based architectural design. The cross-attention is computed between $M$ human part tokens (where $M=16$ is fixed) and $N$ object Gaussian tokens. Unlike standard self-attention which scales quadratically ($O(N^2)$), our cross-attention scales linearly ($O(M \cdot N)$) with respect to the number of object Gaussians. Furthermore, we utilize compact 32-dimensional embeddings for object motion features, which minimizes the memory footprint and matrix multiplication overhead during the forward pass.
}

{
\textbf{Training Cost Justification}.
We acknowledge that our training time ($\sim$5 hours) is longer than the baselines. This is a deliberate trade-off to prioritize physical plausibility and interaction accuracy. Explicitly modeling mutual dependencies and backpropagating gradients through the attention mechanism requires more iterations. However, this cost is strictly confined to the offline training phase, ensuring that the final online user experience remains real-time.
}

\input{tex_Tables/Appendix_object_generation}

\subsection{Additional Ablation Studies}


{
\textbf{Impact of Object Diffusion Prior.} 
To validate the effectiveness of our design choice, we investigate the impact of different geometric priors on the final reconstruction quality. We compare our proposed method, which utilizes a generative Diffusion Prior, against two alternative initialization strategies:\\
(1) MASt3R Prior: Initialization using MASt3R\cite{duisterhof2025mastrsfm}, a state-of-the-art dense matching and reconstruction model. \\
(2) Depth Reconstruction Prior: Initialization using standard monocular metric depth estimation.
}

{
Table \ref{tab:prior_ablation} presents the quantitative comparison on the HOSNeRF dataset. 
Our method equipped with the Diffusion Prior achieves the highest average reconstruction quality (25.89 PSNR), outperforming the MASt3R prior (24.59 PSNR) and the Depth prior (25.36 PSNR).
While discriminative approaches like MASt3R or metric depth estimation rely heavily on visible cues, they often struggle to reconstruct accurate geometry in the presence of heavy occlusions, a common occurrence in human-object interaction scenarios (\textit{e.g.}, hands covering objects).
In contrast, the Diffusion Prior leverages generative knowledge to plausibly complete 3D geometry even in occluded or unseen regions. This holistic geometric initialization provides a more robust starting point for our Cubic Hermite Spline (CHS) deformation, leading to sharper rendering and more stable tracking throughout the dynamic sequence.
}

\subsection{Feature extraction}

\input{tex_FIG/appendix_object_feature}

\textbf{Object feature}.
%우리는 object feature를 추출하기 위해 key frame의 Gaussian에 대해 velocity vector와 임베딩 파라미터를 활용한다. 각 key frame의 velocity vector는 CHS에 적용되어 baseline deformation과 함께 HOI module의 입력 feature로 공동 최적화된다. 추가적으로 각 key frame의 Gaussian마다 29차원의 learnable parameter를 임베딩하며, 이 임베딩은 velocity vector와 결합되어 feature로 사용된다. CHS를 통해 interpolation된 Gaussian feature는 결합된 feature와 time 정보를 입력으로 받아 얕은 MLP layer를 거쳐 projection되며, 최종적으로 32차원의 feature를 형성한다.
As shown in Fig. {\ref{appendix_objfeature}}(a), we extract object features by leveraging the velocity vectors and embedding parameters of Gaussians at key frames. As shown in Fig. {\ref{appendix_objfeature}}(b), each key frame’s velocity vector is applied to the CHS and jointly optimized with the baseline deformation as input features for the HOI module. In addition, a 29-dimensional learnable parameter is embedded for each key frame Gaussian, which is concatenated with the velocity vector to form the feature representation. The interpolated Gaussian features produced by CHS are then combined with the concatenated feature and time information, and projected through a shallow MLP, resulting in a 32-dimensional feature vector.


\textbf{Human feature}.
% Fig. {~\ref{appendix_humanfeature}} illustrates the process of human feature extraction. 
We divide the SMPL-X model into 16 body parts and learn features corresponding to each part. 
Temporal features are sampled from the HexPlane at SMPL-X vertices, where each feature at time $t$ is obtained based on the coordinates $(x_t, y_t, z_t)$. 
For each body part, the features of its associated vertices are averaged to form the part-specific representation $F_{\text{human}}$: 
\[
F_{\text{part}} = \frac{1}{N} \sum_{i \in \text{part}} f_i(x_t, y_t, z_t),
\]
where $N$ denotes the number of vertices belonging to the part. 
As a result, 16 part features, including head, torso, arms, and legs, are obtained and used as inputs to the HOI module. 
This design captures temporally varying dynamic representations while preserving semantically meaningful features for individual body parts.


\subsection{Objective Function Details}
The overall loss function of our model is defined as follows:

\begin{equation}
L = \gamma L_{\text{object motion}} + \beta L_{\text{human}} + \sigma L_{\text{scene}} + L_{\text{depth}},
\end{equation}

where $L_{\text{object motion}}$, $L_{\text{human}}$, and $L_{\text{scene}}$ correspond to losses for object motion, human modeling, and scene context, respectively. The weights $\gamma$, $\beta$, and $\sigma$ control the relative importance of each loss term and are specifically set to 1.0, 0.5, and 0.25, respectively. In our approach, these three terms are optimized simultaneously to consistently model the interactions between humans and objects.

\textbf{Human Loss details} \\
The $L_{\text{human}}$ term consists of losses related to human representation using the SMPL-X (\cite{pavlakos2019expressive}) model. Specifically, it includes the reprojection error between the 3D human joint positions and detected 2D keypoints in images, a mesh-based face loss enhancing the consistency of facial geometry and texture, and a Laplacian regularization term. Additionally, there is an L1 loss ($L_{\text{smplx}}$) between the optimized SMPL-X parameters and the frame-wise initial SMPL-X parameters obtained by a regressor. These loss terms are directly adopted from previous methods such as ExAvatar (\cite{moon2024expressive}), without modifications. For example, the face loss optimizes the consistency between rendered facial images and actual facial images, ensuring geometry-texture coherence. Laplacian regularization is applied to enhance the stability of human body shape. Further details can be found in the referenced research.

Formally, the human loss is given by:

\begin{equation}
L_{\text{human}} = L_{\text{kpt}} + L_{\text{face}} + L_{\text{reg}} + 0.1 \times L_{\text{smplx}},
\end{equation}


% \input{tex_FIG/appendix_HOINetwork}  % COMMENTED OUT - file may be missing
\textbf{Scene Loss details}\\
The $L_{\text{scene}}$ term is a photometric loss focusing on the background regions of the entire scene, following the image similarity-based loss used in existing 3D Gaussian Splatting (\cite{kerbl20233d}) (3DGS) methods. Specifically, a pre-trained human/object segmentation model is employed to mask out human and object regions in the images, optimizing the background Gaussians for the remaining pixels only. This involves minimizing the difference between the rendered result and the background pixels excluding the segmented human and object areas. Occlusions frequently occur during interactions between human hands and objects, causing inconsistencies in masks. By optimizing humans, objects, and backgrounds simultaneously, our method effectively mitigates these boundary inconsistencies.

The scene loss is explicitly defined as:

\begin{equation}
L_{\text{scene}} = 0.8 \times L_1(I_{\text{gt}}, I_{\text{render}}) 
+ 0.2 \times L_{\text{D-SSIM}}(I_{\text{gt}}, I_{\text{render}}),
\end{equation}

\textbf{Object Loss details} \\
The $L_{\text{object}}$ term is a photometric loss that focuses exclusively on the object regions within the scene. We render only the segmented object areas and compute the loss solely on these regions. A pre-trained object segmentation model is employed to isolate object masks in the input images. The object loss encourages accurate reconstruction and appearance consistency for moving objects, which often undergo significant deformation and motion. By supervising only the object regions, this loss helps to refine the geometry and texture of the object-specific Gaussians without being influenced by background or human-related elements.

The object loss is defined as:
\begin{equation}
L_{\text{object motion}} = 0.8 \times L_1(I_{\text{gt}}, I_{\text{obj}}) 
+ 0.2 \times L_{\text{D-SSIM}}(I_{\text{gt}}, I_{\text{obj}}).
\end{equation}


 



==> tex_main/tex_iclr/0_Abstract.tex <==
% \begin{abstract% }
%Reconstructing human-object interaction scenes from monocular videos in the wild remains a significant challenge due to the absence of reliable 3D priors and complex dynamic motions. Existing human-centric reconstruction methods rely heavily on accurate human pose priors and struggle with general dynamic objects, while 4D Gaussian Splatting approaches often fail to capture detailed object motion under occlusion or during long sequences. We present HOIGS, a novel framework that jointly reconstructs humans, dynamic objects, and backgrounds using 3D Gaussians in a unified world space. Our method leverages Score Distillation Sampling (SDS) from a pretrained diffusion model to generate complete 360\textdegree{} 3D shapes at key frames, providing strong geometric priors for initializing dynamic object Gaussians. These priors are temporally propagated using cubic hermite splines, enabling smooth and continuous deformation across time while refining alignment across frames. By combining SMPL-based human modeling, spline-based dynamic object tracking, and Gaussian-based scene representation, HOIGS achieves high-quality reconstruction of complex interaction scenes from monocular inputs. We demonstrate the effectiveness of our approach on challenging real-world sequences, showing substantial improvements over existing baselines in both geometric accuracy and visual fideli% ty.
%\end{abstract}

\begin{abstract}
%인간–객체 상호작용이 포함된 동적 장면을 재구성하는 것은 컴퓨터 비전과 그래픽스 분야의 근본적인 도전 과제이다. 기존 Gaussian Splatting 기반 방법들은 인간 포즈 사전정보에 의존하여 동적 객체를 간과하거나, 모든 움직임을 단일 motion field로 근사하여 복잡한 상호작용을 충분히 포착하지 못한다. 이를 해결하기 위해 본 연구에서는 인간과 객체 간 motion consistency를 명시적으로 학습하는 Human-Object Interaction Gaussian Splatting (HOIGS)를 제안한다. HOIGS는 cross-attention 기반의 HOI 모듈을 통해 사람과 객체의 motion feature 간 상호 의존성을 효과적으로 학습하며, 사람에 대해서는 HexPlane, 객체에 대해서는 Cubic Hermite Spline (CHS)을 deformation baseline으로 적용하여 상호 보완적인 motion feature를 추출한다. 이러한 특징을 통해 HOIGS는 occlusion, contact, manipulation과 같은 복잡한 상호작용 상황에서도 보다 정밀한 deformation 추정을 가능하게 한다. 다양한 데이터셋에서의 실험 결과, 제안한 방법은 기존 human-centric 및 4D Gaussian 접근법을 안정적으로 능가하며, 상호작용 장면의 고품질 재구성을 위한 새로운 가능성을 보여준다.
% Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. To address this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), which explicitly models interaction-induced deformation between humans and objects through a cross-attention based HOI module. Distinct deformation baselines are employed to extract complementary motion features: HexPlane for humans and Cubic Hermite Spline (CHS) for objects. By integrating these heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object manipulation. Comprehensive experiments on multiple datasets demonstrate that our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches, highlighting the importance of explicitly modeling human–object interactions for high-fidelity reconstruction. The video results of HOIGS are available at: \url{https://anonymous.4open.science/w/HOI-GS/}



% Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. To address this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), which explicitly models interaction-induced deformation between a human and multiple objects through a cross-attention based HOI module. Distinct deformation baselines are employed to extract complementary motion features: HexPlane for the human and Cubic Hermite Spline (CHS) for objects. By integrating these heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object manipulation. Comprehensive experiments on multiple datasets demonstrate that our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches. The video results of HOIGS are available at: \url{https://anonymous.4open.science/w/HOI-GS/}



% Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. To address this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), which explicitly models interaction-induced deformation between humans and objects through a cross-attention based HOI module. Distinct deformation baselines are employed to extract complementary motion features: HexPlane for humans and Cubic Hermite Spline (CHS) for objects. By integrating these heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object manipulation. Comprehensive experiments on multiple datasets demonstrate that our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches, highlighting the importance of explicitly modeling human–object interactions for high-fidelity reconstruction. Video results demonstrating the effectiveness of our method are available in the supplementary material.




Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting
methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. To address this gap, we propose Human-Object Interaction Gaussian
Splatting (HOIGS), which explicitly models interaction-induced deformation between humans and objects through a cross-attention based HOI module. Distinct
deformation baselines are employed to extract complementary motion features: HexPlane for humans and Cubic Hermite Spline (CHS) for objects. By integrating these
heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object
manipulation. Comprehensive experiments on multiple datasets demonstrate that
our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches, highlighting the importance of explicitly modeling human–object
interactions for high-fidelity reconstruction. The video results of HOIGS are available at: \url{https://anonymous.4open.science/w/HOIGS-0F47/} 
% Video results demonstrating the effectiveness of our method are available in the supplementary material.
\keywords{Human-Object Interaction (HOI) \and Gaussian Splatting \and Dynamic Scene Reconstruction}




% Reconstructing dynamic scenes with complex human–object interactions is a fundamental challenge in computer vision and graphics. Existing Gaussian Splatting methods either rely on human pose priors, neglecting dynamic objects, or approximate all motions within a single field, limiting their ability to capture interaction-rich dynamics. \textcolor{blue}{To address this gap, we propose Human-Object Interaction Gaussian Splatting (HOIGS), which explicitly models interaction-induced deformation between a human and multiple objects through a cross-attention based HOI module.} \textcolor{blue}{Distinct deformation baselines are employed to extract complementary motion features: HexPlane for the human and Cubic Hermite Spline (CHS) for objects.} By integrating these heterogeneous features, HOIGS effectively captures interdependent motions and improves deformation estimation in scenarios involving occlusion, contact, and object manipulation. \textcolor{blue}{Comprehensive experiments on multiple datasets demonstrate that our method consistently outperforms state-of-the-art human-centric and 4D Gaussian approaches.} \textcolor{blue}{The video results of HOIGS are available at: \url{https://anonymous.4open.science/w/HOI-GS/}}




\end{abstract}

==> tex_main/tex_iclr/1_Introduction.tex <==
\section{Introduction}

%1. 논문에서 다루고자 하는 task (task의 중요성 설명)
% 복잡한 인간–객체 상호작용이 포함된 장면의 비디오를 재구성하고 새로운 시점을 합성하는 것은 컴퓨터 비전과 그래픽스 분야에서 핵심적인 연구 주제이다. 이러한 기술은 가상현실, 메타버스, 3D 애니메이션 등 다양한 응용으로 확장될 수 있다. 그러나 단일 시점 카메라의 한계와 인간–객체 간의 복잡한 상호작용을 정확히 모델링해야 한다는 점은 여전히 고품질 재구성을 위한 주요 도전 과제로 남아 있다. 이러한 문제를 해결하는 것은 실제와 유사한 장면의 이해와 표현을 가능하게 하는 데 필수적이다.

Reconstructing videos of scenes that involve complex interactions between humans and objects and synthesizing novel viewpoints constitute a central research problem in computer vision and graphics. These techniques can be extended to various applications, including virtual reality, the metaverse, and 3D animation. However, the inherent limitations of monocular cameras and the need to accurately model intricate interactions between humans and objects remain major challenges for achieving high-quality reconstruction. Addressing these issues is essential for enabling realistic scene understanding and representation.  


%2. 해당 task의 기존 연구들 -> 문제점을 함꼐 언급하면서 진행

% 2-1 Human 기반의 Gaussian Splatting 기반 문제점을 언급

%최근 사람 중심 비디오 장면 재구성 연구들은 Human Pose Estimation과 Gaussian Splatting을 결합하여 모델링을 수행한다. 일반적으로 각 프레임에 대해 회귀된 SMPL 파라미터를 사전에 획득한 뒤, T-pose를 기준으로 canonical space를 정의하고, 해당 공간에서 3D Gaussian 파라미터를 설정한다. 이후 feature plane과 MLP를 통해 해당 파라미터를 학습하고, LBS(linear blend skinning) 함수를 이용하여 각 프레임에 해당하는 3D 공간으로의 deformation을 적용함으로써 전체 장면을 구성하고 렌더링한다. 이러한 방식은 사람과 배경에 특화된 모델로 발전해왔으며, 정밀한 human pose 정보에 기반해 상대적으로 안정적인 성능을 보인다.
%그러나 기존 접근법들은 사람의 자세 정보를 중심으로 설계되어 있어, 사람과 객체가 동시에 상호작용하는 장면을 직접적으로 모델링하지 못한다. 이로 인해 객체가 동적으로 움직이는 경우에도 정적인 배경으로 처리되거나, 상호작용 과정에서 사람과 객체 간의 관계가 충분히 반영되지 않는 한계가 있다. 따라서 사람과 객체가 함께 상호작용하는 장면을 정확히 재구성하기 위해서는 기존 human-centric 모델을 넘어서는 새로운 모델링 방식이 요구된다.

Recent approaches on human-centric video scene reconstruction (\textcolor{blue}{\cite{kocabas2024hugs,moon2024expressive,hu2024gauhuman,qian20243dgs, liu2024animatable, hu2024gaussianavatar, wen2024gomavatar, kim2025showmak3r}}) have combined human pose estimation with 3D Gaussian Splatting (3DGS) (\textcolor{blue}{\cite{kerbl20233d}}) to model dynamic scenes. Typically, SMPL (\textcolor{blue}{\cite{loper2023smpl}}) parameters are regressed in advance for each frame, and a canonical space is defined using a T-pose as the reference. Within this space, 3D Gaussian parameters are established and trained using feature planes and MLPs. Subsequently, deformation to each frame's 3D space is performed via Linear Blend Skinning (LBS) (\textcolor{blue}{\cite{loper2023smpl}}), allowing for scene reconstruction and rendering. These methods have evolved into specialized models focused on humans and static backgrounds, achieving reliable performance when accurate human pose priors are available. However, existing approaches mainly focus on modeling humans alone, and thus fail to reconstruct complete scenes that involve objects beyond the human body. As a result, dynamically moving objects are often treated as static background or even disappear from the reconstructed scene. Even when deformations of objects are modeled separately, the interactions between humans and objects are not sufficiently considered in dynamic scenarios, which leads to artifacts and noisy results in the interaction regions, as shown in Fig. \textcolor{blue}{\ref{fig:teaser}}. Consequently, accurately reconstructing scenes that involve both humans and objects requires new modeling paradigms that extend beyond conventional human-centric frameworks.

% 2-2 Dynamic scene을 대상으로하흔 Gaussian Splatting의 문제점 언급

%4D Gaussian Splatting 기반 연구들은 사람에 한정되지 않고 임의의 움직이는 객체까지 포괄할 수 있다는 장점이 있으나, 사람 중심 모델에 비해 인간 재구성 성능은 떨어지는 경향이 있다. 이러한 연구들은 대체로 canonical space를 정의하고 이를 world coordinate로 deform하는 implicit function을 학습하거나, 객체의 움직임을 explicit하게 파라미터화하여 학습하는 방식으로 발전하고 있다. 그러나 이러한 접근법들은 객체 간 상호작용을 명시적으로 모델링하지 않고, 모든 움직이는 객체를 단일 motion field로 다루기 때문에 복잡한 interaction을 충분히 반영하지 못한다. 그 결과 implicit 방식은 장기간 혹은 비선형적인 동작을 안정적으로 표현하기 어렵고, explicit 방식은 occlusion, contact, object-to-object dynamics와 같이 interaction에 따라 변화하는 다양한 시나리오를 포괄하기 어렵다.

Recent studies on 4D Gaussian Splatting extend beyond humans to encompass arbitrary moving objects, offering the advantage of general applicability. However, they generally exhibit lower reconstruction performance for humans compared to human-centric models. These approaches typically either define a canonical space and learn an implicit function that deforms it into the world coordinate system (\textcolor{blue}{\cite{wu20244d,jung2023deformable,bae2024per}}), or explicitly parameterize object motions and optimize the corresponding parameters (\textcolor{blue}{\cite{yang2023real,li2024spacetime,lee2024fully}}). Nevertheless, they do not explicitly model interactions between objects and instead treat all moving entities within a single motion field, which limits their ability to capture complex interactions. As a result, implicit methods struggle to represent long-term or highly non-linear motions in a stable manner, while explicit methods fail to handle scenarios such as contact and object manipulation, as ignoring the mutual interactions between motions limits their ability to capture realistic dynamics.

%3. 해당 문제를 해결하기위한 우리의 제안 방법 
%이러한 한계를 극복하기 위해, 우리는 Human-Object Interaction Gaussian Splatting (HOIGS)를 제안한다. HOIGS는 사람과 동적 객체가 동시에 등장하는 복잡한 비디오 장면을 재구성하기 위한 통합 프레임워크로, 기존 접근법이 주로 사람의 움직임만을 모델링했던 것과 달리 사람–객체 간 상호작용을 명시적으로 고려하여 보다 정밀한 deformation 모델링을 가능하게 한다.

%우리 방법의 핵심은 HOI module이며, 이 모듈은 mutual attention 구조를 통해 각 프레임에서 사람의 feature와 객체의 motion feature 간의 양방향 의존성을 학습한다. 구체적으로, 사람의 경우 HexPlane 표현에서 시간에 따라 변화하는 성분을 활용하고, 객체의 경우 keyframe Gaussian의 velocity vector와 관련 파라미터를 임베딩하여 motion feature를 추출한다. 이렇게 얻어진 두 feature를 상호작용하는 attention 구조로 학습함으로써, 기존 연구들이 사람과 객체를 독립적으로 모델링함에 따라 발생했던 artifact나 불안정한 재구성 문제를 효과적으로 해결한다.

%또한, 우리는 사람과 객체 각각에 적합한 deformation baseline을 도입하였다. 객체의 경우, Cubic Hermite Spline (CHS)를 활용하여 연속적인 motion trajectory를 표현하고, keyframe Gaussian의 velocity vector와 추가적인 학습 가능한 파라미터를 결합하여 강건한 motion feature를 형성한다. 사람의 경우에는 HexPlane을 deformation baseline으로 사용하여, 시간적으로 변화하는 파라미터를 공간 feature와 함께 활용함으로써 세밀한 사람의 변형을 효과적으로 모델링한다. 이렇게 추출된 사람과 객체의 feature는 HOI module에 통합되어 각각의 offset vector를 출력하게 되며, 이를 통해 접촉, 조작(manipulation), 복잡한 상호작용 등 다양한 시나리오에서도 정확하고 안정적인 deformation 추정이 가능하다.

To overcome these limitations, we propose Human-Object Interaction Gaussian Splatting (HOIGS), a unified framework for reconstructing complex video scenes that involve both humans and dynamic objects. Unlike previous approaches that either model only human motion or employ a single motion field for all entities, our framework explicitly incorporates human–object interactions to achieve more faithful deformation modeling.

% \textcolor{blue}{
% We introduce deformation baselines tailored to the distinct characteristics of humans and objects. For humans, we employ SMPL-X-based Gaussian modeling to achieve robust representation against occlusions and detailed deformation. By combining temporally varying parameters with spatial features, we effectively model fine-grained human deformation while maintaining inter-frame consistency. For objects, we apply Cubic Hermite Spline (CHS) to smoothly represent continuous motion trajectories, forming robust motion feature representations by combining velocity vectors of keyframe Gaussians with learnable auxiliary parameters.
% }
% \textcolor{blue}{
% Finally, we design a Cross-Attention-based HOI module to reflect interaction intensity between humans and multiple objects. Extracted human features and object features exchange information complementarily through cross-attention, generating interaction features. Subsequently, through MLP heads, Gaussian mean offsets are predicted for objects, while SMPL-X pose offsets are predicted for humans. This interaction-based attention architecture enables accurate and stable deformation estimation across diverse scenarios including artifacts, contact, manipulation, occlusion, and complex interactions that arise when modeling humans and objects independently.
% }
At the core of our framework lies the HOI module, which adopts a mutual attention mechanism to capture the bidirectional dependencies between human features and object motion features at each frame. Specifically, the module receives temporally varying human features, derived from the dynamic components of the HexPlane representation, together with object motion features, obtained by embedding velocity vectors and their associated parameters. By explicitly learning how these two types of features influence one another, the HOI module effectively overcomes the shortcomings of prior methods that modeled humans and objects independently, which often resulted in artifacts and unstable reconstructions in interaction-rich scenes.

Furthermore, we design different deformation baselines tailored to humans and objects. For objects, we employ the Cubic Hermite Spline (CHS) to capture continuous motion trajectories, embedding the velocity vectors of keyframe Gaussians along with additional learnable parameters to construct robust object motion features. For humans, we utilize HexPlane as the deformation baseline, where time-varying parameters are leveraged to represent fine-grained human deformation in both spatial and temporal domains. The extracted features from both humans and objects are subsequently integrated within the HOI module, which outputs offset vectors for each entity. This design ultimately enables our framework to achieve accurate and stable deformation estimation, even under complex scenarios involving close contact, mutual manipulation, or other intricate human–object interactions.

In summary, our main contributions are as follows:

\begin{itemize}
 
    \item We propose an entity-aware cross-attention HOI module that enforces motion consistency between humans and objects. By attending to their features, it captures interdependent dynamics and improves reconstruction during contact and manipulation.
        
    \item We design distinct strategies for humans and objects using tailored deformation baselines. HexPlane encodes temporal and spatial features for human motion, while Cubic Hermite Splines (CHS) embed velocity vectors and learnable parameters for objects. This separation enables accurate and expressive motion representations for both entities.

    \item We conduct extensive experiments on diverse human–object interaction scenes and demonstrate that our method achieves more accurate reconstruction compared to existing human-centric and 4D Gaussian approaches.

\end{itemize} 

==> tex_main/tex_iclr/2_Relatedwork.tex <==
\section{Related Works}

\subsection{Human Modeling}

%Research on modeling realistic human has been actively pursued for a long time. Initially, parametric models were proposed, and based on these, the Human Mesh Reconstruction (HMR) model (\textcolor{blue}{\cite{kanazawa2018end}}) was introduced for estimating human poses from a single image. However, although these models offer computational efficiency, they remain limited in their ability to represent non-body parts such as clothing and accessories. To overcome this limitation, implicit function-based methods (\textcolor{blue}{\cite{huang2020arch, saito2019pifu, saito2020pifuhd, xiu2022icon, xiu2023econ}}) were proposed. While this line of work is capable of capturing fine details such as clothing and hair, it remains limited in ensuring global consistency and achieving efficient rendering performance. These methods place their primary focus on reconstructing human geometry, with limited consideration of HOI aspects. With the emergence of Neural Radiance Fields(NeRF) (\textcolor{blue}{\cite{mildenhall2021nerf}}), several approaches (\textcolor{blue}{\cite{peng2021neural, jiang2022neuman, weng2022humannerf, alldieck2022photorealistic, liao2023high, guo2023vid2avatar}}) applying NeRF to human body modeling were introduced. Despite their strengths in view consistency and realistic appearance modeling, NeRF-based methods remain limited by high computational training costs and inefficient rendering performance. In terms of HOI, certain work (\textcolor{blue}{\cite{fan2024hold}}) attempted to incorporate objects into the scene. Nevertheless, the treatment of objects was still constrained, as their dynamic properties and more general forms of human–object interaction were not fully captured. Recently, a new 3D representation method called 3D Gaussian Splatting (3DGS) (\textcolor{blue}{\cite{kerbl20233d}}) was proposed. There have also been attempts to apply it to 3D human reconstruction (\textcolor{blue}{\cite{kocabas2024hugs, moon2024expressive, hu2024gauhuman,  liu2024animatable, hu2024gaussianavatar}}).
%In these works. they primarily focused on animatable and efficient representations of the human body, while objects appearing in the scene were still regarded as static and non-interactive. To address this issue, a method that leverages cross-interaction between human and objects in dynamic HOI scenes is required. Therefore, we propose the HOIGS model which achieves stable human reconstruction in dynamic scenes and effectively models HOI.


Research on realistic human modeling has long been pursued. Early parametric models enabled efficient estimation of human pose, exemplified by HMR (\textcolor{blue}{\cite{kanazawa2018end}}), but struggled to capture clothing and accessories. To address this, implicit function-based methods (\textcolor{blue}{\cite{huang2020arch, saito2019pifu, saito2020pifuhd, xiu2022icon, xiu2023econ}}) were proposed, which recover fine details such as hair and clothing but remain limited in global consistency and rendering efficiency. These methods mainly focused on human geometry with little attention to human-object interactions. With Neural Radiance Fields (NeRF) (\textcolor{blue}{\cite{mildenhall2021nerf}}), several works applied it to human modeling (\textcolor{blue}{\cite{peng2021neural, jiang2022neuman, weng2022humannerf, alldieck2022photorealistic, liao2023high, guo2023vid2avatar}}), achieving realistic appearance and view consistency but still suffering from high training cost and slow rendering. In terms of human-object interactions, some attempts (\textcolor{blue}{\cite{fan2024hold}}) introduced objects, yet dynamic interactions were not fully captured. Recently, 3D Gaussian Splatting (3DGS) (\textcolor{blue}{\cite{kerbl20233d}}) emerged as a new representation and has been applied to human reconstruction (\textcolor{blue}{\cite{kocabas2024hugs, moon2024expressive, hu2024gauhuman, liu2024animatable, hu2024gaussianavatar}}). However, most efforts still regard objects as static. 
Recent approaches leverage multi-view data for high-fidelity results. For example, Animatable Gaussian \cite{li2024animatable} and GASPACHO \cite{mir2025gaspacho} utilize multi-view setups to create relightable avatars and disentangle human-object interactions. However, these methods depend on complex capture settings, whereas real-world scenarios are predominantly monocular. To address this, we propose HOIGS, a model for stable human reconstruction that explicitly captures human–object interactions from monocular inputs.




% To achieve high-fidelity animation and interaction, recent approaches have leveraged multi-view data settings. For instance, Animatable Gaussian \cite{li2024animatable} employs multi-view RGB videos to reconstruct a parametric template and uses 2D CNNs to predict pose-dependent Gaussian maps for creating realistic, relightable avatars. Furthermore, GASPACHO \cite{mir2025gaspacho} extends multi-view 3DGS to complex scenarios, explicitly reconstructing humans and objects as separate Gaussian sets to enable controllable interaction synthesis under significant occlusions. However, these methods rely on multi-view setups for accurate tracking and template reconstruction, whereas real-world capture is predominantly monocular. To overcome this, we propose HOIGS, a model for stable human reconstruction in dynamic scenes that explicitly captures human–object interactions.}



% Research on realistic human modeling has long been pursued. Early parametric models enabled efficient estimation of human pose, exemplified by HMR (\textcolor{blue}{\cite{kanazawa2018end}}), but struggled to capture clothing and accessories. To address this, implicit function-based methods (\textcolor{blue}{\cite{huang2020arch, saito2019pifu, saito2020pifuhd, xiu2022icon, xiu2023econ}}) were proposed, which recover fine details such as hair and clothing but remain limited in global consistency and rendering efficiency. These methods mainly focused on human geometry with little attention to human-object interactions.
% With Neural Radiance Fields (NeRF) (\textcolor{blue}{\cite{mildenhall2021nerf}}), several works applied it to human modeling (\textcolor{blue}{\cite{peng2021neural, jiang2022neuman, weng2022humannerf, alldieck2022photorealistic, liao2023high, guo2023vid2avatar}}), achieving realistic appearance and view consistency but still suffering from high training cost and slow rendering. In terms of human-object interactions, some attempts (\textcolor{blue}{\cite{fan2024hold}}) introduced objects, yet dynamic interactions were not fully captured.
% Recently, 3D Gaussian Splatting (3DGS) (\textcolor{blue}{\cite{kerbl20233d}}) emerged as a new representation and has been applied to human reconstruction (\textcolor{blue}{\cite{kocabas2024hugs, moon2024expressive, hu2024gauhuman, liu2024animatable, hu2024gaussianavatar}}). However, most efforts still regard objects as static. To overcome this, we propose HOIGS, a model for stable human reconstruction in dynamic scenes that explicitly captures human–object interactions. 


\subsection{Dynamic Scene Modeling}
The field of dynamic scene rendering and reconstruction has seen a paradigm shift from initial NeRF-based methods  (\textcolor{blue}{\cite{park2021nerfies, park2021hypernerf, wu2022d, fridovich2023k}}) to the more recent 3D Gaussian Splatting framework. Previous studies such as HOSNeRF (\textcolor{blue}{\cite{liu2023hosnerf}}) effectively modeled human-object interactions by controlling human motion through skeleton-based models such as SMPL and leveraging object state embeddings. Nevertheless, the implicit representation inherent to NeRF led to significant computational overhead in training and rendering, and limited the ability to represent detailed features in large-scale environments. To address this efficiency bottleneck, a line of work has emerged that extends 3DGS to the temporal domain, known as 4D Gaussian Splatting (4DGS) (\textcolor{blue}{\cite{wu20244d, yang2023real}}). Although these methods achieve real-time rendering speeds, they face persistent issues. Most 4DGS approaches rely on Structure-from-Motion for Gaussian initialization, which is fundamentally ill-suited for dynamic subjects as it operates on the assumption of a static world. This leads to inaccurate point cloud generation for moving objects. Moreover, the MLP-based implicit deformation fields used to capture motion, while adequate for simple trajectories, often result in over-smoothed or unnatural movements when applied to complex, in-the-wild scenarios. Therefore, we propose an explicit, spline-based motion model. This approach allows us to model intricate temporal movements with high fidelity, achieving high-quality rendering even in dynamic scenes that include complex human-object interactions.


==> tex_main/tex_iclr/4_Method.tex <==
\input{tex_FIG/Method_main_fig}

\section{Method}
% 
% method 개요 설명
%우리는 사람과 객체의 deformation을 각각 독립적으로 모델링한 뒤, HOI 모듈을 통해 상호작용에 따른 변형을 반영하여 최종적으로 장면을 재구성한다. 먼저 객체의 deformation은 Cubic Hermite Spline을 통해 추정한다. 사람의 deformation은 HexPlane feature를 기반으로 하며, 시간에 대해 불변한 spatial feature를 활용하여 canonical space에 정의된 T-pose의 texture를 학습하고, 이후 Linear Blend Skinning(LBS)을 통해 각 world space로 deformation을 적용한다. 이러한 deformation baseline을 통해 사람과 객체를 각각 모델링하며 각 프레임에 대한 대략적인 위치를 추정한 뒤, 그로부터 motion feature를 추출한다. 마지막으로, 추출된 human과 object feature를 HOI 모듈에 입력하여 두 객체 간 상관관계에 따른 변형을 고려하고, 이를 통해 최종적으로 interaction 장면에서의 사람과 객체의 위치를 결정한다. 
As shown in Fig. \textcolor{blue}{~\ref{figure_main_method}}, we reconstruct the scene by independently modeling the deformations of humans and objects, and then incorporating interaction-aware transformations through the HOI module. Object deformations are estimated using a Cubic Hermite Spline (CHS). Human deformations are based on HexPlane features, where time-invariant spatial features are used to learn the texture of the canonical T-pose, and Linear Blend Skinning (LBS) is subsequently applied to deform the canonical representation into each world space. Using these deformation baselines, we independently model humans and objects and estimate their approximate positions for each frame, from which motion features are extracted. Finally, the extracted human and object features are fed into the HOI module, which accounts for interaction-driven transformations and determines the final positions of humans and objects in the reconstructed interaction scene.
\subsection{Object deformation}
% 우리는 diffusion prior와 SDS loss를 적용하여 전체 시퀀스를 대표하는 프레임에서 객체를 재구성한다. 재구성된 객체는 각 키프레임의 카메라 파라미터를 이용해 warping을 수행함으로써, 해당 키프레임의 3D Gaussian을 초기화한다% .
%Diffusion prior를 통해 생성된 3D Gaussian은 실제 물체의 형상과 다소 차이가 있을 수 있다. Diffusion은 그럴듯한 이미지를 기반으로 3D shape을 생성할 수 있으나, 실제 물체의 형상을 정확하게 복원하지는 못한다. 이에 우리는 diffusion 기반으로 생성된 초기 3D shape을 실제 물체의 형상 및 기하 정보와 정합시키기 위해, explicit한 3D Gaussian deformation 모델을 도입% 한다.
%key frame들로 warping된 Gaussian $G_k$의 mean 값 $\mathbf{m}$과 color 값만을 추출하고, 나머지 3D Gaussian 파라미터는 identity 값으로 초기화한다. 우리는 key frame에서 새롭게 정의된 mean과 color를 기반으로 object의 3D Gaussians을 구성하고, 이를 통해 object의 deformation을 모% 델링한다.
%Object의 시간에 따른 연속적인 움직임을 표현하기 위해, 각 Gaussian의 mean 값을 제어점 기반의 곡선으로 모델링한다. 이를 위해 Cubic Hermite Spline 기반의 함수 $CHP(t, \mathbf{m})$를 정의하고, 시간 $t$에서의 object Gaussian의 위치 $M(t)$를 다음과 같이 추정한다:
% $M(t)=CHP(t, m)$ 
% 여기서 $\mathbf{m} = \left{ \mathbf{m}_k \mid \mathbf{m}k \in \mathbb{R}^3 \right}{k \in [0, N_c - 1]}$는 key frame들의 mean 위치들로 구성된 learnable한 제어점 집합이며, $N_{key}$는 제어점의 개수를 나타낸다.
% $CHP(t, m)$은 다음과 같이 수식화된다:
%수식
% notation설명.
%$m_{\lfloor t_s \rfloor}$는 $\lfloor t_s \rfloor$번째 key frame에 해당하는 3D Gaussian의 mean 값을 의미한다.
%기존의 spline 정의에서 tangent는 단순히 보간을 위한 기울기로 사용되지만, 우리는 이를 velocity로 해석하여 motion feature로 활용한다. 즉, 각 Gaussian mean의 시간에 따른 위치 변화율을 velocity vector로 정의하고, 이를 임베딩함으로써 객체의 motion feature를 구성한다. 이렇게 얻어진 velocity 기반 motion feature는 객체의 동적인 움직임을 보다 효과적으로 표현할 수 있다.
% Key frame 사이의 위치 파라미터 $m$은 각 key frame에 존재하는 Gaussian의 위치 $m_k$를 기반으로 Spline을 이용해 추정된다. 학습되는 Gaussian들은 key frame에 대응되는 Gaussian들로, key frame 사이의 Gaussian은 추정된 후 렌더링되고, 손실 함수를 통해 계산된 gradient가 역전파되어 해당 key frame의 Gaussian 파라미터가 업데이트된다.
% Gaussian 파라미터 중 rotation과 opacity는 시간에 따라 변화하는(time-dependent) 파라미터로 설정하였다. Rotation은 각 key frame에서의 Gaussian rotation 값을 기반으로 Spherical Linear Interpolation(Slerp)을 적용하여 시간에 따른 연속적인 변화를 모델링하였다. Opacity는 물체의 움직임에 따라 발생하는 occlusion 영역을 반영할 수 있도록 time 값에 따라 변화하도록 설계하였다. 한편, scale 파라미터는 모든 key frame에서 대응되는 Gaussian들에 대해 동일한 값으로 고정하였다.
\textcolor{blue}{\noindent\textbf{Object Initialization.}
We begin by segmenting the object of interest and cropping the object region from a representative frame of the entire sequence. Next, we apply a diffusion model initialized from DreamScene4D~\cite{dreamscene4d} and guided by SDS loss to generate a canonical 3D Gaussian point cloud of the object. However, the 3D Gaussians generated through this diffusion prior may differ from the actual object geometry. While diffusion models can generate plausible 3D shapes from images, they often fail to precisely recover the true object structure. To address this, we align the diffusion-based canonical 3D Gaussians with the world space. First, we estimate a per-frame warping scale $S_t$ by minimizing the discrepancy between the projected 3D bounding box and the 2D mask bounding box for each frame $t$.
We then compute the global scale $S$ as the average over all frames:}

\[
S_t = \arg\min_{S_t} \left\| \text{BBox}_{\text{proj}}(S_t \cdot \text{Gaussians}) - \text{BBox}_{\text{mask}}^t \right\|, \quad
S = \frac{1}{T} \sum_{t=1}^{T} S_t .
\]
\textcolor{blue}{
where $T$ is the total number of frames. We then transform the scaled Gaussians to the world coordinate system using the COLMAP camera extrinsics $R_t$ and $\mathbf{t}_t$ as follows:}

\[
\mathbf{x}_{\text{world}}^t = R_t^{-1} (\mathbf{x}_{\text{cam}}^t - \mathbf{t}_t).
\]

From the warped Gaussians $G_k$ of each keyframe, we extract each Gaussian’s mean and color value, while initializing the remaining 3D Gaussian parameters with identity values.

\textcolor{blue}{\noindent\textbf{\noindent\textbf{Object Deformation.}}} \
Based on the redefined mean and color from the keyframes, we construct the object’s 3D Gaussians and use them to model the object deformation. To represent the continuous motion of the object over time, we model the mean values of each Gaussian as control-point-based curves. Specifically, we define a Cubic Hermite Spline function $\text{CHS}(t, \mathbf{m})$, and estimate the position of an object Gaussian at time $t$, denoted as $\mathbf{M}(t)$, as follows:

\noindent This initialization ensures that the explicit 3D Gaussian deformation model aligns with the actual object geometry and structural information. 
From the warped Gaussians of each keyframe, we extract each Gaussian’s mean and color value, while initializing the remaining 3D Gaussian parameters with identity values.
We apply a diffusion prior with SDS loss to reconstruct the object from a representative frame of the entire sequence. The reconstructed object is then warped using the camera parameters of each keyframe to initialize the corresponding 3D Gaussians.
However, the 3D Gaussians generated through the diffusion prior may differ from the actual object geometry. While diffusion models can generate plausible 3D shapes from images, they often fail to precisely recover the true object structure. To address this, we introduce an explicit 3D Gaussian deformation model that aligns the diffusion-based initialization with the actual object geometry and structural information.
From the warped Gaussians $G_k$ of each keyframe, we extract each Gaussian's mean and color value, while initializing the remaining 3D Gaussian parameters with identity values. Based on the redefined mean and color from the keyframes, we construct the object’s 3D Gaussians and use them to model the object deformation.
To represent the continuous motion of the object over time, we model the mean values of each Gaussian as control-point-based curves. Specifically, we define a Cubic Hermite Spline function $CHS(t, \mathbf{m})$, and estimate the position of an object Gaussian at time $t$, denoted as $M(t)$, as follows:
\[
M(t) = CHS(t, \bold{m}),
\]
where $\bold{m} = \left\{ m_k \mid m_k \in \mathbb{R}^3 \right\}_{k \in [0, N_{key} - 1]}$ is a learnable set of control points representing the mean positions of the Gaussians at each key frame, and $N_{key}$ denotes the number of key frames. $CHS(t, \mathbf{m})$ is formulated as

\vspace{-2mm}

\begin{equation}
\begin{aligned}
CHS(t, \mathbf{m}) &= (2t_r^3 - 3t_r^2 + 1)m_{\lfloor  t_s  \rfloor} + (t_r^3 - 2t_r^2 + t_r)\tau_{\lfloor t_s \rfloor  } \\
&\quad + (-2t_r^3 + 3t_r^2)m_{\lfloor t_s  \rfloor + 1} + (t_r^3 - t_r^2)\tau_{\lfloor t_s \rfloor  + 1}, 
\end{aligned}
\end{equation}

where $t_r = t_s - \lfloor t_s  \rfloor $, $t_s = t_n (N_{key} - 1)$, $t_n = \frac{t}{N_f - 1}$ and $N_f$ denotes the number of all frames.
$m_{\lfloor t_s \rfloor}$ denotes the mean of the 3D Gaussians corresponding to the $\lfloor t_s \rfloor$-th key frame.

In the standard formulation, $\tau_{\lfloor t_s \rfloor}$ represents the tangent vector with respect to the means of the surrounding Gaussians, which is typically approximated as $\tau_{\lfloor t_s \rfloor} = \tfrac{1}{2}\left(m_{\lfloor t_s \rfloor+1} - m_{\lfloor t_s \rfloor-1}\right)$. Instead of using this fixed approximation, we reinterpret $\tau_{\lfloor t_s \rfloor}$ as a \textit{velocity vector} and employ it as a learnable parameter. By embedding this velocity, we construct motion features that better capture the dynamic behavior of objects over time.

The position parameter $\bold{m}$ between key frames is estimated via spline interpolation using both the Gaussian positions $m_k$ at the key frames and the corresponding velocity vectors $\tau_{ \lfloor k \rfloor }$. Only the Gaussians at the key frames are directly optimized during training. Once the intermediate Gaussians are estimated and rendered, the resulting gradients from the loss function are backpropagated to update the parameters of the corresponding key frame Gaussians.
Among the Gaussian parameters, rotation and opacity are defined as time-dependent variables. The rotation parameter is modeled using Spherical Linear Interpolation based on the Gaussian rotations at each key frame, enabling smooth transitions over time. The opacity parameter varies with time to account for occluded regions caused by object motion. In contrast, the scale parameter is kept constant across all corresponding Gaussians at different key frames.
\subsection{Human deformation}
\textcolor{blue}{\noindent\textbf{\noindent\textbf{HexPlane-based Deformation.} }} \
% \noindent\textbf{HexPlane-based Deformation.} \
We model human deformation using HexPlane features. 
Specifically, we adopt time-invariant spatial features $f$ from HexPlane to learn the texture of the canonical T-pose mesh $T_c$ in the canonical space. The features $f$ are processed by an MLP head $\psi$ to learn the Gaussian properties in the canonical space. This representation serves as the baseline for human deformation. The canonical human representation is then deformed into the posed world space using Linear Blend Skinning (LBS) as follows:
\begin{equation}
\psi_h(f(T_c)) = (c, o, \Delta P_c, R, S, W),
\end{equation}
\begin{equation}
P_{def} = \alpha * LBS(P_c , \theta, W),
\end{equation}
where $\theta$ denotes the set of SMPL-X pose parameters and $\alpha$ is a learnable scale parameter for human pose. 
Equation (3) extracts the Gaussian properties (color $c$, opacity $o$, position offset $\Delta P_c$, rotation $R$, scale $S$ and skinning weights $W$) from the canonical HexPlane features, 
while Equation (4) applies the LBS function to obtain the deformed positions $P_{def}$ of the Gaussians in the posed space. 

To ensure that the reconstructed human representation matches the actual geometry, 
we further apply a depth supervision loss:
\begin{equation}
\mathcal{L}_{depth} = \left\| D_{render} - D \right\|_1,
\end{equation}
where $D_{render}$ is the rendered depth map from the deformed Gaussians and $D$ is the depth obtained from an off-the-shelf metric depth estimation model and further scaled using the COLMAP point cloud. 
This depth-guided supervision constrains the learnable scale parameter $\alpha$ and improves geometric fidelity in the reconstructed human shape.

\textcolor{blue}{\subsection{Cross-Attention Interaction Module}}
\textcolor{blue}{\textbf{Feature Extraction.}} We extract time-varying features from both humans and objects to learn their interactions. For humans, instead of relying on time-invariant texture features from the canonical space, we utilize time-varying features from HexPlane. Furthermore, since it is not possible to know in advance which body parts are involved in object interactions, we divide the human body into 16 parts and extract HexPlane features for each part.

For objects, the features are derived from the velocity embeddings associated with each keyframe in the deformation process, which capture the local motion information at those frames. In addition, we embed learnable parameters for each keyframe to represent latent motion characteristics that cannot be fully captured by velocity alone. These velocity vectors and learnable parameters are then projected together with the corresponding time values, enabling the construction of object motion features. This formulation allows us to obtain continuous motion features for objects across all frames, rather than being limited to discrete keyframes.


% Before

% \textbf{HOI module.} The proposed HOI module takes time-varying features of humans and objects as inputs and explicitly models their interactions. 
% Let the human and object features be denoted as $F_{\text{Human}}$ and $F_{\text{Object}}$. 
% To capture interdependencies between the two, we apply \textit{mutual attention}, where queries, keys, and values are defined as:
% \begin{equation}
% Q_h = F_{\text{Human}}W_h^Q,\;\; K_o = F_{\text{Object}}W_o^K,\;\; V_o = F_{\text{Object}}W_o^V,
% \end{equation}
% \begin{equation}
% Q_o = F_{\text{Object}}W_o^Q,\;\; K_h = F_{\text{Human}}W_h^K,\;\; V_h = F_{\text{Human}}W_h^V.
% \end{equation}

% Cross-attention is then performed in both directions, from human to object and from object to human, while incorporating a distance mask $B$ into the attention computation:
% \begin{equation}
% A_{h \leftarrow o} = \text{softmax}\!\left(\tfrac{Q_hK_o^\top}{\sqrt{d}} + B\right),\quad
% A_{o \leftarrow h} = \text{softmax}\!\left(\tfrac{Q_oK_h^\top}{\sqrt{d}} + B^\top\right).
% \end{equation}

% This process yields updated features $F'_{\text{Human}}$ and $F'_{\text{Object}}$ that embed interaction cues. 
% Finally, $F'_{\text{Human}}$ is used to regress $\Delta$SMPL-X refinements (body pose, hand pose, translation), while $F'_{\text{Object}}$ is used to predict $\Delta G_{\text{object}}$, i.e., corrections for Gaussian-based object motion. 
% In this way, the HOI module augments the baseline deformations (HexPlane+LBS for humans and CHS for objects) with interaction-aware adjustments, enabling accurate reconstruction of human--object interaction scenes.



% \begin{equation}
% Q_h = F_{\text{Human}}W_h^Q,\;\; K_o = F_{\text{Object}}W_o^K,\;\; V_o = F_{\text{Object}}W_o^V,
% \end{equation}
% \begin{equation}
% Q_o = F_{\text{Object}}W_o^Q,\;\; K_h = F_{\text{Human}}W_h^K,\;\; V_h = F_{\text{Human}}W_h^V.
% \end{equation}

\textcolor{blue}{\textbf{Interaction Module.}} \textcolor{blue}{The proposed Interaction module (HOI module)} takes time-varying features of humans and objects as inputs and explicitly models their interactions. 
Let the human and object features be denoted as $F_{\text{Human}}$ and $F_{\text{Object}}$. 
To capture interdependencies between the two, we apply \textit{mutual attention}, where queries, keys, and values are defined as:
\begin{equation}
\begin{aligned}
Q_h, K_h, V_h &= F_{\text{Human}}W_h^Q,\; F_{\text{Human}}W_h^K,\; F_{\text{Human}}W_h^V, \\
Q_o, K_o, V_o &= F_{\text{Object}}W_o^Q,\; F_{\text{Object}}W_o^K,\; F_{\text{Object}}W_o^V.
\end{aligned}
\end{equation}
Cross-attention is then performed in both directions, from human to object and from object to human, while incorporating a distance mask $B$ into the attention computation:
\begin{equation}
F'_{\text{Human}} = \text{softmax}\!\left(\tfrac{Q_hK_o^\top}{\sqrt{d}} + B\right)V_h,\quad
F'_{\text{Object}} = \text{softmax}\!\left(\tfrac{Q_oK_h^\top}{\sqrt{d}} + B^\top\right)V_o.
\end{equation}




\textcolor{blue}{The distance mask $B$ filters out distant objects based on their 3D spatial proximity to the human.
Specifically, for each object, we compute the Euclidean distance between the object's Gaussian center $c_{\mathrm{obj}}^{\mathrm{world}}$ and the human pelvis position $p_{\mathrm{pelvis}}^{\mathrm{world}}$ in world coordinates. 
$B_{ij}$ encodes the relative distance between the $i$-th human token and the $j$-th object token:}

\begin{equation}
B_{ij} = \begin{cases}
-\infty & \text{if } \lVert c_{\mathrm{obj}}^{\mathrm{world}} - p_{\mathrm{pelvis}}^{\mathrm{world}} \rVert \ge \tau \\
0 & \text{otherwise}
\end{cases},
\end{equation}
 
\textcolor{blue}{where $\tau$ is set to the human arm length (derived from the SMPL-X model). When $B_{ij}=-\infty$, the corresponding object tokens are masked out during attention, effectively excluding non-interacting background objects.}

This process yields updated features $F'_{\text{Human}}$ and $F'_{\text{Object}}$ that embed interaction cues. 
Finally, $F'_{\text{Human}}$ is used to regress $\Delta$SMPL-X refinements (body pose, hand pose), while $F'_{\text{Object}}$ is used to predict $\Delta G_{\text{object}}$, i.e., corrections for Gaussian-based object motion. 
In this way, the HOI module augments the baseline deformations (HexPlane+LBS for humans and CHS for objects) with interaction-aware adjustments, enabling accurate reconstruction of human--object interaction scenes.






% \begin{equation}
% A_{h \leftarrow o} = \text{softmax}\!\left(\tfrac{Q_hK_o^\top}{\sqrt{d}} + B\right),\quad
% A_{o \leftarrow h} = \text{softmax}\!\left(\tfrac{Q_oK_h^\top}{\sqrt{d}} + B^\top\right).
% \end{equation}

% \textcolor{blue}{\textbf{Interaction Module.}} \textcolor{blue}{The proposed Interaction module (HOI module)} takes time-varying features of humans and objects as inputs and explicitly models their interactions. 
% Let the human and object features be denoted as $F_{\text{Human}}$ and $F_{\text{Object}}$. 
% To capture interdependencies between the two, we apply \textit{mutual attention}, where queries, keys, and values are defined as:

% \begin{equation}
% \begin{aligned}
% Q_h, K_h, V_h &= F_{\text{Human}}W_h^Q,\; F_{\text{Human}}W_h^K,\; F_{\text{Human}}W_h^V, \\
% Q_o, K_o, V_o &= F_{\text{Object}}W_o^Q,\; F_{\text{Object}}W_o^K,\; F_{\text{Object}}W_o^V.
% \end{aligned}
%
% \end{equation}


% Cross-attention is then performed in both directions, from human to object and from object to human, while incorporating a distance mask $B$ into the attention computation:


% \begin{equation}
% F'_{\text{Human}} = \text{softmax}\!\left(\tfrac{Q_hK_o^\top}{\sqrt{d}} + B\right)V_h,\quad
% F'_{\text{Object}} = \text{softmax}\!\left(\tfrac{Q_oK_h^\top}{\sqrt{d}} + B^\top\right)V_o.
% \end{equation}

% This process yields updated features $F'_{\text{Human}}$ and $F'_{\text{Object}}$ that embed interaction cues. 
% Finally, $F'_{\text{Human}}$ is used to regress $\Delta$SMPL-X refinements (body pose, hand pose, translation), while $F'_{\text{Object}}$ is used to predict $\Delta G_{\text{object}}$, i.e., corrections for Gaussian-based object motion. 
% In this way, the HOI module augments the baseline deformations (HexPlane+LBS for humans and CHS for objects) with interaction-aware adjustments, enabling accurate reconstruction of human--object interaction scenes.






\subsection{Optimization}
% Canonical space에 정의된 T-pose 형태의 human Gaussian, 배경 Gaussian, 그리고 움직이는 객체에 대한 dynamic motion을 공동으로 최적화함으로써, human-object interaction 상황을 효과적으로 재구성한다. 우리는 기존 Human Gaussian Splatting 방법과 유사하게, 각 프레임에 대해 SMPL 파라미터를 regression하고, 모든 프레임에 공통으로 대응되는 T-pose 형태의 human canonial space에 정의한다. 이 canonial human을 기반으로 3D Gaussian 파라미터는 feature plane과 MLP를 통해 추정되며, 해당 파라미터는 texture가 표현된 공간을 구성한다. 이후 각 프레임의 회귀된 SMPL 파리미터를 바탕으로, LBS(Linear Blend Skinning)를 통해 canonical Gaussian들이 해당 프레임으로 deformation된다. 우리는 ExAvatar에서 영감을 받아, body shape뿐만 아니라 얼굴과 손의 표현까지 확장하기 위해 SMPL-X 모델을 사용하였다. 배경은 3D Gaussian Splatting 기반으로 표현된다.


% We reconstruct the final human-object interaction scenario by jointly optimizing the T-pose Gaussians defined in a canonical space, background Gaussians, and dynamic motion modeling for moving objects. Similar to existing human Gaussian Splatting approaches\cite{moreau2024human, li2024animatable, kocabas2024hugs, moon2024expressive, hu2024gauhuman, qian20243dgs}, we regress the SMPL parameters\cite{loper2023smpl} for each frame and define a canonical T-pose human shared across all frames. The 3D Gaussian parameters in the canonical space are predicted using a feature plane and an MLP, forming a textured space. These canonical Gaussians are then deformed to each frame using the regressed SMPL parameters via Linear Blend Skinning (LBS)\cite{loper2023smpl}. Inspired by ExAvatar\cite{moon2024expressive}, we adopt SMPL-X\cite{pavlakos2019expressive} to represent not only the body shape but also fine-grained facial and hand motions. The background is separately modeled using standard 3D Gaussian Splatting\cite{kerbl20233d}.

% 방금 언급한 human과 backgroud에 대한 모델, 그리고 object가 함께 최적화 되어지는 모습을 보이기!
% 사용된 loss들 전부 언급하고, loss를 통해 3D Gaussian들이 어떻게 global minimum을 찾아가는지를 기입

% 최적화 과정은 각가 독립적으로 분리되는 것이 아닌, 한번에 1-stage 로 함께 학습이 진행된다.
% 우리는, 객체, 인간, 배경을 동시에 모델링한다.
% 배경은 일반적인 3DGS( 3d gaussian splatting )을 사용하여, 모델링이 되었다.
% 학습에는 객체와 사람 영역 마스킹을 통해, 배경만을 분리하여, 정적 가우시안 배경이 photometric loss 를 통해 학습되었다.
% 사람 모델링의 경우, 기존에 존재하는 일반적인 접근 방법처럼, feature plane 기반 가우시안 모델링을 하였으며, 객체와 함께 상호작용하는 자연스러운 모델링을 위해, SMPL-X 기반 모델 아바타 모델을 사용하였다.
% 전 프레임에 대해, SMPL-X 파라미터를 추출하고, Canonical T-pose human avatar 를 정의해, LBS 변환을 통해 각 프레임에 변형시켰다.
% 학습 과정에는 가우시안 랜더러를 통해 나온 결과와 인간 영역을 비교하는 이미지 손실 기반 (SSIM,LPIPS,L1) 손실이 사용되었다. 자세한 내용은 부록에 기술하였다.
% \textbf{객체 시작 최적화}
% 객체는 SDS Loss 를 사용해 객체 모델링이 되었다. 객체 모델링에 있어서, 전체 프레임에서 객체를 마스킹을 통해 분리하고, 해당 객체를 diffusion을 통해 고해상도 3d 모델링을 한다.  학습에서 특정 카메라 뷰를 제한해 optimazation 과정이 안정화 되도록 하였다.

For background modeling, we employ the standard 3D Gaussian Splatting (3DGS) technique. During training, we isolate the background by masking out the object and human regions, allowing the static Gaussian background to be optimized using a photometric loss. For human modeling, \textcolor{blue}{we regress the SMPL-X parameters by \cite{moon2022accurate}}, and incorporate an SMPL-X-based avatar model to ensure natural interaction with the object. For each frame, we extract the SMPL-X parameters and define a canonical T-pose human avatar. This canonical avatar is then deformed to match each frame using LBS. During training, image-based loss metrics such as SSIM, LPIPS, and L1-norm were utilized to compare the Gaussian renderer's output with the human region in the image. 

\textbf{Object Motion Optimization}. We model the motion of objects using CHS to ensure continuity in position interpolation. A CHS is a piecewise cubic polynomial that is defined by both the positions and the first derivatives (tangents) at key points in time. By specifying the starting and ending slopes for each spline segment, CHS guarantees smooth transitions between key frames, maintaining continuity not only in the object’s position but also in its velocity. In other words, the object’s trajectory over time remains continuous and smooth, without abrupt jumps or changes in speed. This property is crucial for accurately modeling temporal motion in a realistic and stable manner.

\textbf{Integrated Optimization}.
% 통합 최적화
We train our model using an integrated optimization objective that combines multiple loss terms. Specifically, the overall loss function is formulated as:
\[
\mathcal{L} = \gamma \, \mathcal{L}_{\text{object motion}} + \beta \, \mathcal{L}_{\text{human}} + \sigma \, \mathcal{L}_{\text{scene}} + \mathcal{L}_{\text{depth}},
\]
where $\mathcal{L}_{\text{object motion}}$, $\mathcal{L}_{\text{human}}$, and $\mathcal{L}_{\text{scene}}$ are the loss components for the object's motion, the human-related factors, and the scene context, respectively. Here, $\gamma$, $\beta$, and $\sigma$ are hyperparameters that control the relative weight of each loss term during training. By tuning these hyperparameters, we balance the influence of each component on the training objective. This integrated optimization approach ensures that the model simultaneously accounts for object motion accuracy, human interaction plausibility, and scene consistency during learning.


==> tex_main/tex_iclr/5_Experiments.tex <==
\section{Experiments}

\subsection{Implementation Details}
We use ExAvatar (\textcolor{blue}{\cite{moon2024expressive}}) as the baseline human rendering model, and all hyperparameters are kept identical to those used in ExAvatar. For object deformation using splines (\textcolor{blue}{\cite{ahlberg2016theory, de1978practical}}), we fix the time interval to 4 for all scenes. Training is conducted using an NVIDIA H100 GPU, taking approximately 5 hours per scene.
\vspace{-5pt}
\subsection{Datasets}
\textbf{HOSNeRF dataset (\textcolor{blue}{\cite{liu2023hosnerf}}).} We use the monocular dynamic-scene dataset HOSNeRF, which captures human–object interaction scenarios. The dataset comprises recordings in six indoor and outdoor locations with six subjects interacting with objects within a single scenario. Each sequence contains 300–400 frames. For evaluation, we uniformly select 16 frames per sequence for testing and use the remaining frames for training, following HOSNeRF.

\textbf{BEHAVE dataset (\textcolor{blue}{\cite{bhatnagar2022behave}}).} We use the BEHAVE multi-view RGB-D human–object interaction dataset, but adapt it to a monocular setting by selecting a single fixed camera from the four static viewpoints for each sequence. Specifically, we curate 9 sequences covering four distinct indoor environments, five subjects, and four objects. From each sequence’s raw video, we uniformly sample 300 frames. For evaluation, we uniformly select 16 frames per sequence for testing and use the remaining frames for training 

\textbf{ARCTIC dataset (\textcolor{blue}{\cite{fan2023arctic}}).} We use the ARCTIC hand–object interaction dataset and extend comparisons to hand–object baselines. Since HOIGS is human-centric rather than hand-only, we evaluate only sequences where the full body is visible. Specifically, we use sequences of one subject interacting with four objects. Each monocular sequence (≈600 frames) is split by uniformly sampling 16 frames for testing and using the rest for training.


\input{tex_FIG/Experiments_hosnerf}
\input{tex_FIG/Experiments_behave}
\input{tex_FIG/Experiments_arctic}
\input{tex_Tables/HOSNeRF_dataset}
\input{tex_Tables/BEHAVE_dataset}
\input{tex_Tables/ARCTIC_dataset}

\subsection{Qualitative results}

We compare our view-synthesis results with existing Gaussian-based models, which generally outperform NeRF-based methods in rendering quality. The experimental results are visualized in Fig. ~\textcolor{blue}{\ref{fig:visual_HOSNeRF}}. The dynamic-scene models D3DGS (\textcolor{blue}{\cite{yang2024deformable}}) and Ex4DGS (\textcolor{blue}{\cite{lee2024fully}}) yield ghosting artifacts for both human and dynamic objects because they fail to disentangle human and object motions within complex interactions. ExAvatar (\textcolor{blue}{\cite{moon2024expressive}}) reconstructs humans but does not handle dynamic objects. Our method accurately reconstructs humans and objects with temporally coherent motion, using CHS object trajectories with velocity vectors and the human backbone based on HexPlane and LBS, while the HOI module further ensures contact consistency. On the ARCTIC dataset, as shown in Fig.~\textcolor{blue}{\ref{fig:visual_ARCTIC}}, HOLD (\textcolor{blue}{\cite{fan2024hold}}) shows limited performance in full-body–object interactions, whereas HOIGS successfully reconstructs them. This is because HOLD reconstructs only hands, while HOIGS reconstructs the entire human body including the hands. On the BEHAVE dataset, as shown in Fig.~\textcolor{blue}{\ref{fig:visual_BEHAVE}}, whereas ExAvatar suffers body–background overlap due to human misalignment in world space, our depth-based alignment ensures accurate human placement. Through qualitative results, we further confirm that our method effectively reconstructs complex human–object interactions with visually consistent outcomes.


\subsection{Quantitative results}
As shown in Tab.~\textcolor{blue}{\ref{tab:hosnerf_comparison}}, HOIGS achieves the highest PSNR and the lowest LPIPS on the Backpack, Tennis, Suitcase, Dance, and Lounge scenarios of the HOSNeRF dataset, surpassing prior 3D Gaussian-based models in visual quality. Tab.~\textcolor{blue}{\ref{tab:BEHAVE_comparison}} shows that on the BEHAVE dataset, it likewise attains the highest PSNR and lowest LPIPS, demonstrating effective reconstruction of complex human–object interactions from single-view input. Tab.~\textcolor{blue}{\ref{tab:ARCTIC_comparison}} shows that on the ARCTIC dataset, our method outperforms the hand–object model HOLD  (\textcolor{blue}{\cite{fan2024hold}}). Unlike HOLD, our model reconstructs complex full-body geometry while simultaneously capturing interactions with dynamic objects.



\subsection{Ablation study}

\input{tex_Tables/ablation}
We conduct ablation studies to validate the effectiveness of the proposed method. As shown in Tab.~\textcolor{blue}{\ref{ablation}}, modeling object deformation with a simple MLP yields the lowest performance, while our CHS-based baseline deformation improves PSNR by 0.5, demonstrating its superiority. Removing the HOI module and applying only velocity further results in a 0.6 drop in PSNR compared to the full model, confirming the necessity of explicitly modeling human–object interactions. Finally, replacing the time-varying HexPlane features with simple parameter embeddings for the human features leads to a 0.2 decrease in PSNR, highlighting the effectiveness of our human feature design.

==> tex_main/tex_iclr/6_Conclusion.tex <==
\section{Conclusion}
We presented HOIGS, a novel framework for reconstructing dynamic scenes with explicit modeling of human–object interactions from monocular videos. By combining HexPlane-based human deformation, spline-based object motion, and an interaction-aware HOI module, our method achieves stable and accurate reconstruction even in challenging scenarios with contact and manipulation. In particular, the explicit treatment of human-object interactions enables our framework not only to recover realistic human geometry but also to faithfully capture object dynamics and their mutual influences, which have been largely overlooked in prior works. Extensive experiments on HOSNeRF, BEHAVE, and ARCTIC datasets demonstrate that HOIGS outperforms state-of-the-art human-centric and 4D Gaussian approaches in both visual quality and consistency, highlighting its effectiveness in advancing realistic modeling of complex human–object interactions.

\textbf{Limitations and future works.} While our framework handles typical dynamic motions well, it struggles under minimal camera movement, where COLMAP-based pose and point cloud estimation becomes unreliable. This often leads to rendering artifacts. Future work may improve robustness in such low-baseline settings by jointly optimizing camera poses during training.


% 사람에 대해서 novel pose가 주어질 경우, 새로운 장면을 만들 수 있다. 다만, 객체에 대해서는 사람에 종속적으로 영향을 받는 연구가
